Simpler is More: Efficient Top-K Nearest Neighbors Search on Large Road Networks

Top-k Nearest Neighbors (kNN) problem on road network has numerous applications on location-based services. As direct search using the Dijkstra's algorithm results in a large search space, a plethora of complex-index-based approaches have been proposed to speedup the query processing. However, even with the current state-of-the-art approach, long query processing delays persist, along with significant space overhead and prohibitively long indexing time. In this paper, we depart from the complex index designs prevalent in existing literature and propose a simple index named KNN-Index. With KNN-Index, we can answer a kNN query optimally and progressively with small and size-bounded index. To improve the index construction performance, we propose a bidirectional construction algorithm which can effectively share the common computation during the construction. Theoretical analysis and experimental results on real road networks demonstrate the superiority of KNN-Index over the state-of-the-art approach in query processing performance, index size, and index construction efficiency.

==> approach_old.tex <==
\section{Index Construction $\&$ Update}
\label{sec:indexcon}

Based on the structure of \knnindex, it can be constructed straightforwardly by computing the top $k$ nearest neighbors of each vertex through \kw{Dijkstra's} algorithm or \emph{TEN-Index}. However, these approaches are time-consuming  (with time complexity  $O(n \cdot (m + n \cdot \log n ))$ or $O(n \cdot \log n + n \cdot h \cdot w + n \cdot h \cdot k)$ ). Obviously, these approaches are unscalable to handle large road network. In this section, we present our new approach to construct the \knnindexcnt.

\subsection{Main Ideas and Overview of Our Approach}
\label{sec:mi}


The above discussed approaches compute the $k$ nearest neighbors for each vertex independently, which misses the potential opportunities to re-use the intermediate results during the construction. In this section, we introduce important observations regarding the essential vertex set and shortest distance computation, which lays the foundation of our computation-sharing index construction algorithm.

%\begin{definition}
%    \textbf{($u$ Vertex set)}
%	\label{def:ev}
%	Given a graph $G$, for a vertex $u$, a subset of vertices $\vc(u) \subset V(G)$ is a vertex set for $u$ if $u$ disconnects with any vertices of the graph $V(G)\setminus\{\vc(u) \cup \{u\}\}$ after removing $\vc(u)$ from $G$. 
%\end{definition}

%\begin{example}
%	Following this definition, $\nbr(u)$ is a vertex set for $u$. Since after deleting $\nbr(u)$, $u$ cannot connect with other vertices in the original graph $G$. For $v_{12}$, $\vc(v_{12}) = \{ v_3, v_4, v_5, v_{11}, v_{18} \}$.
%\end{example}

\begin{definition}
    \textbf{($u$ Essential Vertex Set)}
	\label{def:ev}
	%Given a graph $G$, for a vertex $u$, if for $\forall w \in \ev(u)$, the weight of the edge $(u,w)$ is equal to their shortest distance in $G$, we call $\ev(u)$ as an essential vertex set for $u$, namely, $\ev(u) = \{ w | w \in \nbr(u) \wedge \phi(u,w) = \sd(u,w) \}$. 
	Given a graph $G$, for a vertex $u$, if for $\forall w \in \ev(u)$, $w \in \spath(u,v)$ for each $v \in G$, we call $\ev(u)$ as an essential vertex set for $u$. %, namely, $\ev(u) = \{ w | w \in \nbr(u) \wedge \phi(u,w) = \sd(u,w) \}$.
	
	%Given a graph $G$, for a vertex $u$, a subset of vertices $\ev(u) \subset V(G)$ is an essential vertex cut for $u$. For each vertex $w$ in $\ev(u)$, shortest path between $u$ and every vertex $v$ in $G$ must pass through $w$ at least once. Namely, for each edge $(u,v) \in G$ such that $\phi(u,v) = \sd(u,v)$.
\end{definition}

\begin{example}
	In \reffig{roadnetwork}, we take $v_8$ as an example. We can see $\nbr(v_8) = \{ v_2, v_6, v_7, v_{20}, v_9 \}$. The shortest path between $v_8$ and $v_9$ is $(v_8, v_{20}, v_9)$, the shortest distance is $\sd(v_8,v_9) = 3$, which is not equal to the weight of edge $\phi(v_8,v_9) = 5$. $\sd(v_8,v_9) \neq \phi(v_8,v_9)$. So $v_9$ does not belong to $\ev(v_8)$. Similarly, we can conclude that $v_6$ and $v_7$ also does not belong to $\ev(v_8)$. For the graph $G$ in \reffig{roadnetwork}, an essential vertex set of $v_8$ is $\ev(v_8) = \{ v_2, v_{20} \}$.
\end{example}

There is only an example to explain \refdef{ev}. Our essential vertex set generation for each vertex is not only to delete some neighbors from its original neighbor set via deleting unsatisfied edges. Details will be illustrated in \refsec{evs}.

Based on \refdef{ev}, we have following properties for the essential vertex set and $k$ nearest neighbors for:

\begin{property}
	\label{pro:vcknn}
	Given a road network $G$, an essential vertex set $\ev(u)$ for $u$, let $\knnalg(u)$ denotes $k$ nearest neighbors for $u$, we have:
	
	\hspace{5em}$\knnalg(u) \subseteq \cup_{w \in \vc(u)} \knnalg(w)$.
\end{property}
	
\proofsketch
	We prove this property by contradiction. We assume that $v \in \knnalg(u)$ but $v \notin \cup_{w \in \vc(u)} \knnalg(w)$. According to \refdef{ev}, the shortest path $\spath(u,v)$ must pass through at least one vertex $w \in \vc(u)$ such that for all $v_i \in \knnalg(w)$, $1 \leq i \leq k$, we have $dist(w,v_i) < dist(w,v)$. Then $dist(u, w) + dist(w,v_i) < dist(u,w) + dist(w,v)$. It means there are at least $k$ vertices whose distance to $u$ is smaller than the distance between $u$ and $v$, which contradicts $v \in \knnalg(u)$. The proof completes.
\eop

Based on this observation, we have the following property regarding the distance computation to select top $k$ vertices as $\knnalg(\cdot)$: 

\begin{property}
\label{pro:sd}
     Given a road network $G$, an essential vertex set $\ev(u)$ for $u$, let $\knnalg(u)$ be $k$ nearest neighbors for $u$, $\forall v \in \knnalg(u)$, we have:
	 \begin{equation}
	 	\label{eq:sdcomp}
	 	\sd(u,v) = min_{ w \in \ev(u)} \{ \sd(u,w) + \sd(w,v) \}.
	 \end{equation}
\end{property}

\proofsketch
	According to \refdef{ev}, for $\forall v \in \knnalg(u)$, each shortest path between $u$ and $v$, $\spath(u,v)$, must pass through at least one vertex $w \in \ev(u)$, so $\sd(u,v) = \sd(u,w) + \sd(w,v)$. \refeq{sdcomp} is tenable.
\eop

%In other words, if we have known $\knnalg(w)$ for each vertex $w \in \ev(u)$, we can know the relatively small candidate set of $\knnalg(u)$.

As analysed in \refpro{vcknn}, for a vertex $v$, if $v \in \knnalg(u)$, $v$ must be in $\cup_{w \in \ev(u)} \knnalg(w)$. Following \refpro{sd}, given an essential vertex set $\ev(u)$ for $u$, precomputed the distance between $u$ and each vertex $w \in \ev(u)$ and its $\knnalg(w)$, for each $v \in \cup_{w \in \ev(u)}\knnalg(w)$ we can calculate $\sd(u,v)$ efficiently. Then, after sorting $\sd(u,v)$ in an ascending distance order, the set of top $k$ vertices, $\knnalg(u)$, can be obtained. Therefore, after achieving $\ev(u)$, $\sd(u,w)$ and $\knnalg(w)$ for every vertex $w$ in $\ev(u)$, it is ready to compute $\knnalg(u)$. 

However, prior to computing $\knnalg(u)$, it is non-trival to generate $\ev(u)$ and to compute distance between $u$ and each vertex $w \in \ev(u)$. And it is impossible to compute $\knnalg(w)$ without independence. To increase dependency for \knnindex construction of each vertex, we assign a rank for each vertex. In \reffig{roadnetwork}, we rank all vertices via their ID. Then according to the rank, we compute $k$NN for each vertex. For $v_1$, since each vertex in its essential vertex set $\ev(v_1)$ has not been calculated, we only can use Dijkstra's Algorithm to grab $k$NN without any distance re-use. Then for $v_2$, $v_1 \in \ev(v_2) = \{ v_1, v_8 \}$ and we can use \refpro{sd} to calculate the "distance" between $v_2$ and $v \in \knnalg(v_2)$ via $v_1$. However, $v_2$ still needs to use Dijkstra's Algorithm to grab exact $k$NN, since the "distance" can not be confirmed as the shortest distance. Here, we adopt a parital-then-complete strategy to construct \knnindex with making full use of \refpro{vcknn} and \refpro{sd}. Next, we will introduce the overview of our approach to use above properties well. %To avoid computing $\knnalg(u)$ individually, we 


\stitle{Overview of Our Approach.} Based on above analysis, our approach consists of two parts. The first one is to construct $\ev(u)$ for each vertex $u \in V$ and compute the distance between $u$ and each vertex $w \in \ev(u)$. We achieve the essential vertex sets and those distance via obtaining Shortest Distance Preserved Graph \sdg from the input graph $G$. The second part is how to construct \knnindex based on \sdg via the parital-then-complete strategy in \refsec{ug}. Furthermore, we propose an improved \knnindex construction with the assistance of the existing computed labels in \refsec{utl}.

%Our approach consists of two parts. First one is to construct $\ev(u)$ for each vertex $u \in V$ and compute the distance between $u$ and each vertex $w \in \ev(u)$. We construct Local Distance Preserved Graph \textbf{\ldg} to generate a rank order for all vertices and add new edges to avoid distance computation between each vertex with its lower rank vertices repeatedly. The neighbor set of each vertex in \ldg is sufficient but probably redundant to be used as essential vertex set. To further achieve essential vertex sets, we transform \textbf{\ldg} to Shortest Distance Preserved Graph \textbf{\sdg} via deleting unnecessary edges \refsec{evs}. The second part is how to construct \knnindex based on \sdg via the parital-then-complete strategy in \refsec{ug}. Furthermore, we propose an improved \knnindex construction with the assistance of the existing computed labels in \refsec{utl}.

%\stitle{A Naive \knnindex Construction Method.} As analysed above, it is easy to think about using \kw{Dijkstra's} algorithm to calculate $\knnalg(w)$ for $\forall v \in \vc(u)$ first and then re-using computed distance to calculate $\knnalg(u)$ directly based on \refpro{vcknn} and \refpro{sd}.

\subsection{Essential Vertex Sets and Distance}
\label{sec:evs}
%\stitle{Drawbacks of the Naive Method.} Next, we discuss the drawbacks of the naive solution in terms of time complexity:

%\begin{enumerate}
%	\item \kw{Dijkstra's} algorithm wastes too much time. when the size of the candidate object set is small, the worst case is to explore all vertices in the whole graph.
%	\item The Distance re-use rate is too low. Even if we can re-use part of computed \knnindex, the Distance re-use rate is too low in the part of \kw{Dijkstra's} algorithm searching. Relatively, the above naive method is still calculated independently.
%\end{enumerate}

%CH \cite{geisberger2008contraction},
In order to design an efficient algorithm to construct the \knnindexcnt, we first introduce the concept of the shortest distance preserved graph.

\begin{definition}
	\label{def:sdg}
	\textbf{(SD-Graph)} Given a road network $G$, a graph $G_{SD}$ is its \underline{S}hortest \underline{D}istance Preserved Graph \stitle{(SD-Graph)} such that for each edge $\forall (u,v) \in E(G_{SD})$, $\phi((u,v), G_{SD}) = \sd((u,v),G)$. And $V(G_{SD}) = V(G)$.
\end{definition}

%To avoid Dijkstra and maximize times of distance re-use, we adopt graph reduction\cite{bodlaender2006treewidth} to add new edges to the original input graph to avoid a part of Dijkstra and to achieve vertex sets. As a by-product, we can get a \stitle{rank} $\pi(\cdot)$ for all vertices in $G$. Here, we denote $\pi(u)$ as \stitle{$\rank(u)$} for each vertex $u$ in $G$. Different from graph reduction\cite{bodlaender2006treewidth}, when we reduce the graph, simultaneously we retain the old graph $G$ with updated weight and new added edges in $G'$. %We define $G'$ as \underline{L}ocal \underline{D}istance Preserved Graph \stitle{(LD-Graph)}. For each vertex $u$ in $G'$, we set $\vc(u) = \nbr'(u)$. $nbr'(u)$ is the neighbor set for $u$ in $G'$, denoted as $\nbr'(u) = \{ v | (u,v) \in G' \}$.

%$G'$ is the \stitle{(LD-Graph)} of the input graph $G$. For each vertex $u$ in $G'$, we set $\vc(u) = \nbr'(u)$. $nbr'(u)$ is the neighbor set for $u$ in $G'$, denoted as $\nbr'(u) = \{ v | (u,v) \in G' \}$.


%\begin{algorithm}[htb]
%        \caption{Vertex Set and \ldg Generation}
%        \label{alg:vsgen}
%        \DontPrintSemicolon
%        \KwInput{A road network $G$}
%        \KwOutput{LD-Graph $G'$}
%        $G' \gets G$; $i \gets 1$; \;
%        \While{$V(G) \neq \emptyset$}{
%        	$w \gets$ the vertex with smallest degree in $V(G)$; \;
%        	\ForAll{pairs of vertices $u,v \in \nbr(w,G)$}{
%               	\If{$(u,v) \notin E(G)$}{
%               		insert $(u,v)$ into $G'$ and $G$;\;
%               		$\phi'(u,v) \gets \phi'(u,w) + \phi'(w,v)$; \;
               		%$\phi_{G'}(u,v) \gets \phi_{G'}(u,w) + \phi_{G'}(w,v)$; \;
%            		}\ElseIf{$\phi'(u,w) + \phi'(w,v) < \phi'(u,v)$}{
            		%}\ElseIf{$\phi_{G'}(u,w) + \phi_{G'}(w,v) < \phi_{G'}(u,v)$}{
%                		$\phi'(u,v) \gets \phi'(u,w) + \phi'(w,v)$; \;
%            		}
%        	}
%        	remove all edges connected to $w$ in $G$; \;
%        	$\pi(w) \gets i$; $i \gets i+1$; \;
%        }
        %\ForAll{$u \in G'$}{
        %	$\vc(u) \gets \nbr'(u)$;
        %}
%\end{algorithm} 

%\begin{definition}
%	\label{def:vp}
%	\textbf{(Valley Path)}\cite{wei2020architecture} A path $\vpath(v_1,v_l) = (v_1,v_2,...,v_l)$ between $v_1$ and $v_l$ is defined as a \stitle{valley path}, if $\pi(v_i) < min \{ \pi(v_1), \pi(v_l) \}$, for $\forall i \in [2,l-1]$; that is, any intermediate vertex of $p$ has a lower rank than the endpoints.
%\end{definition}

% We denote the valley path with shortest distance between $u$ and $v$ as $\vspath(u,v)$, also called as shortest valley path between $u$ and $v$. And we denote the distance of $\vspath(u,v)$ as $\vsd(u,v)$, shortest valley distance.

%\begin{definition}
%	\label{def:ld}
%	\textbf{(LD-Graph)} Given a road network $G$, a graph $G_{LD}$ is its \underline{L}ocal \underline{D}istance Preserved Graph \stitle{(LD-Graph)} such that for each edge $\forall (u,v) \in E(G_{LD})$, $\phi((u,v), G_{LD}) = \vsd(u,v)$. And $V(G_{LD}) = V(G)$, $ E(G) \subseteq E(G_{LD})$.
%\end{definition}




%\stitle{Vertex sets and \ldg Generation.} Given a graph $G$ and a vertex set $V(G)$, the vertex set generating operation for each vertex $w$ in $G$ transforms the input graph $G$ into \ldg $G'$ in \refalg{vsgen} as follows: the vertex $w$ with the smallest degree in $G$ is chose in line 3. For every pair of neighbors $(u,v)$ of $w$ in $G$, if $(u,v) \notin E(G)$, a new edge $(u,v)$ with weight $\phi'(u,v) = \phi'(u,w)+\phi'(v,w)$ is inserted into $G$ and $G'$. Otherwise, if $\phi'(u,v)+\phi'(v,w) < \phi'(u,w)$, the weight of edge $(u,v)$ in $G'$ is updated as $\phi'(u,v)+\phi'(v,w)$. Then, all edges connected to $w$ in $G$ are removed in line 10. Here, we only need to add edges without weight into $G$, since $G$ is used to keep the structure of the original graph and to maintain the original graph's connectivity. $G'$ is used to record new added edges and the edges with updated weights. $\phi'(\cdot,\cdot)$ represents each edge's weight in $G'$. Definitely, those new added edges and updated weights sufficiently avoid \kw{Dijkstra's} algorithm search from each vertex to vertices connected with its neighbors with lower ranks. In line 11, we assign a rank $i$ to the chose vertex $w$, and the rank counter plus 1. % graph reduction alg should be in the appendix



%A path $\vpath(v_1,v_l) = (v_1,v_2,...,v_l)$ between $v_1$ and $v_l$ is defined as a \stitle{valley path}\cite{wei2020architecture} if $\pi(v_i) < min \{ \pi(v_1), \pi(v_l) \}$, for $\forall i \in [2,l-1]$; that is, any intermediate vertex of $p$ has a lower rank than the endpoints. We denote the valley path with smallest distance between $u$ and $v$ as $\vspath(u,v)$, also called as the shortest valley path between $u$ and $v$. And we denote the distance of $\vspath(u,v)$ as $\vsd(u,v)$, shortest valley distance. Below \reflem{svd} proofs that in the \ldg $G'$, for each edge $(u,v)$ such that $\phi'(u,v) = \vsd(u,v)$. Above new add edges are shortest valley paths, each edge's weight is equal to its shortest valley distance. 

%\begin{figure}
%    \centering
%    \includegraphics[width=0.80\linewidth]{fig1/PG.pdf}
%    \vspace{-0.2cm}
%    \caption{LD-Graph of $G$}
%    \label{fig:PG}
%\end{figure}

%\begin{example}
%	\reffig{PG} shows \ldg for the road network $G$ in \reffig{roadnetwork}. As shown in \reffig{PG}, for valley paths between $v_{17}$ and $v_{20}$, one valley path $P_1 = (v_{17}, v_{16}, v_{20})$, the second valley path $P_2 = (v_{17}, v_{15}, v_{10}, v_{14}, v_{20})$ and $P_3 = (v_{17}, v_{15}, v_{14}, v_{20})$. Since the distance of these valley paths $P_2$ and $P_3$ is smallest, $\vsd(v_{17},v_{20}) = 9$, $\vspath(v_{17},v_{20}) = P_2$ (or $P_3$).
%\end{example}

%\begin{lemma}
%	\label{lem:svd}
%	Given a graph $G$, after achieving its LD-Graph $G'$, the weight of each edge $(u,v)$ is equal to the shortest valley distance between $u$ and $v$, namely, $\phi'(u,v) = \vsd(u,v)$.
%\end{lemma}

%\proofsketch
%	There are two cases for $\phi'(u,v)$ computation:
%	\begin{itemize}
%		\item Case 1: $\phi'(u,v) = \phi(u,v)$. Definitely, this case shows that $\vspath(u,v) = \{u,v\}$.
%		\item Case 2: $\phi'(u,v) \neq \phi(u,v)$, which means that there is a valley path between $u$ and $v$, $vpath(u,v)$. Line 8 in \refalg{vsgen} shows that when we meet every valley path between $u$ and $v$, we only save the smaller one. At the end, the smallest one is saved. New added edges also can be explained in this case. For each new added edge $(u,v)$, we can think $\phi(u,v) = +\infty$.
	%\end{itemize}
%	Overall, in \ldg $G'$ of $G$, $\phi'(u,v)$ denotes shortest valley distance between $u$ and $v$. If there is a shortest valley path for each pair of vertices $u,v$, the edge $(u,v)$ must exist in \ldg. 
%\eop

%\begin{theorem}
%	\label{thm:ldg}
%	\textbf{Time Complexity Analysis.} The time complexity of vertex set and \ldg generation in \refalg{vsgen} is bounded by $O(n \cdot (f^2 + log(n)))$. Here, $f = max_{w \in G}|\vc(w)|$.
%\end{theorem}

%\proofsketch
%	In \refalg{vsgen}, each vertex in the graph will be scanned in lines 2-11. Line 3 needs $O(log(n))$ to the vertex with smallest degree by binary search. Adding edges and updating weight costs $O(f^2)$ (Lines 4-9). In the lines 12-13, we scan each vertex in the graph to achieve $\vc(\cdot)$ bounded by $O(n)$. Overall, the time complexity is $O(n \cdot(f^2 + log(n)))$.
%\eop

%Recall \refpro{sd}, for $\forall v \in \knnalg(u)$, $\sd(u,v)$ is calculated via two parts. The first part is the shortest distance from $u$ to the vertex $w$ such that $w \in \vc(u)$. The second part is the shortest distance from $w$ to $v$. $\sd(w,v)$ will be solved in \refsec{utl}. Here, we focus on the first part and notice that in \ldg $G$ the weight of edge between $u$ and $w$ may not be equal to the shortest distance between $u$ and $w$, namely, $\phi(u,w)$ ?= $\sd(u,w), \forall w \in \vc(u)$. To maximize distance re-use rate, we first make sure that $\phi(u,w) = \sd(u,w), \forall w \in \vc(u)$. For the edge $(u,w)$, whose weight $\phi(u,w) \neq \sd(u,w)$, we delete it to narrow down our computation scale. Definitely, smaller the size of vertex set for each vertex in the graph $|\vc(\cdot)|$ is, lower the KNN construction time complexity is. We will explain the details in \refthm{tc_utl}. 


% the way they compute shortest distance between XXX and XXX via a top-down manner. For our work,  

Inspired by \cite{wei2010tedi}, we adopt a reversing order of $\pi(\cdot)$ to check whether $\phi(u,v)$ is equal to $\sd(u,v)$. Next, we will introduce the lemma about how to check:

\begin{lemma}
	\label{lem:sdcheck}
	Given a graph $G$ and its \ldg $G'$, for each edge $(u,v) \in G'$, if $\phi'(u,v) = \sd(u,v)$, there does not be any $w \in \nbr^+(u)$ with $\phi'(u,w) + \phi'(w,v) < \phi'(u,v)$. Here, $\nbr^+(u) = \{v | v \in \nbr'(u) \wedge \pi(v) > \pi(u)\}$.
\end{lemma}

\proofsketch
	There are two cases for checking $\phi'(u,v)$ in $G'$:
	\begin{itemize}
		\item Case 1: $\phi'(u,v) = \sd(u,v)$, namely, $\vsd(u,v) = \sd(u,v)$. Here, there are two sub-cases: (1) $\phi(u,v) = \phi'(u,v)$, which denotes that $\spath(u,v) = \vspath(u,v) = \{u,v\}$. (2) $\phi(u,v) \neq \phi'(u,v)$, which means that there exists a shortest valley path $\vspath(u,v) = \spath(u,v)$ such that $\vsd(u,v) = \sd(u,v)$. In this case, when shortest path is also a shortest valley path, there will not exit a vertex $w \in \nbr^+(u)$ such that $\phi'(u,w) + \phi'(w,v) < \phi'(u,v)$. %According to \reflem{svd}, after generating \ldg, $\phi'(u,v)$ is $\vsd(u,v)$. So there is not any $w \in \nbr^+(u)$ such that $\phi'(u,w) + \phi'(w,v) < \phi'(u,v)$.
		\item Case 2: $\phi'(u,v) \neq \sd(u,v)$, namely, $\vsd(u,v) \neq \sd(u,v)$. The shortest valley path between $u$ and $v$ is not the shortest path $u$ and $v$, so $\spath(u,v)$ must pass through one neighbor $w \in \nbr^+(u)$. There is at least one vertex $w \in \nbr^+(u)$ such that $\phi'(u,w) + \phi'(w,v) < \phi'(u,v)$. 
	\end{itemize}
	Overall, for any edge $(u,v)$ in $G'$, if $\phi'(u,v) = \sd(u,v)$, for $\forall w \in nbr'(u)$, $\phi'(u,w) + \phi'(w,v) >= \phi'(u,v)$.
\eop

\begin{figure}[htb]
 \vspace{-0.1cm}
  \centering
   \subfigcapskip=0pt
   \subfigcaptopadj=0pt
   \subfigure[Check $v_{10}$]
   	 { \includegraphics[width=0.46\linewidth]{fig1/check10.pdf}
       \label{fig:CH_10}}
 \subfigure[Check $v_{17}$]{ \includegraphics[width=0.46\linewidth]{fig1/check17.pdf}
 	   \label{fig:CH_17}
	 }
  \vspace{-0.1cm}
 \caption{Checking Procedure for $v_{10}$ and $v_{17}$}
  \label{fig:check1}
\end{figure}


%\begin{figure}[htb]
% \vspace{-0.1cm}
%  \centering
%   \subfigcapskip=0pt
%   \subfigcaptopadj=0pt
%   \subfigure[Check $v_{10}$]
%   	 { \includegraphics[width=0.35\linewidth]{fig1/CK10.pdf}
%       \label{fig:CH_10}}
% \subfigure[Check $v_{15}$]{ \includegraphics[width=0.4\linewidth]{fig1/CK15.pdf}
 %	   \label{fig:CH_15}
%	 }
 % \vspace{-0.1cm}
 %\caption{Checking Procedure for $v_{10}$ and $v_{15}$}
 % \label{fig:check}
%\end{figure}

Before introducing our check procedure, we first introduce the following definition:



\begin{algorithm}[htb]
        \caption{Essential Vertex Sets and \sdg Generation}
        \label{alg:evgen}
        \DontPrintSemicolon
        \KwInput{A road network $G$, a total vertex rank $\pi$}
        \KwOutput{\sdg $G'$}
        %$G' \gets G$; $i \gets 1$; \;
        %\While{$V(G) \neq \emptyset$}{
        \ForEach{$w$ in the order $\pi$}{
        	%$w \gets$ the vertex with smallest degree in $V(G)$; \;
        	\ForAll{pairs of vertices $u,v \in \nbr(w,G)$}{
               	\If{$(u,v) \notin E(G)$}{
               		insert $(u,v)$ into $G$;\;
               		$\phi'(u,v) \gets \phi'(u,w) + \phi'(w,v)$; \;
               		%$\phi_{G'}(u,v) \gets \phi_{G'}(u,w) + \phi_{G'}(w,v)$; \;
            		}\ElseIf{$\phi'(u,w) + \phi'(w,v) < \phi'(u,v)$}{
            		%}\ElseIf{$\phi_{G'}(u,w) + \phi_{G'}(w,v) < \phi_{G'}(u,v)$}{
                		$\phi'(u,v) \gets \phi'(u,w) + \phi'(w,v)$; \;
            		}
        	}
        	%remove all edges connected to $w$ in $G$; \;
        	%$\pi(w) \gets i$; $i \gets i+1$; \;
        }
        $G' \gets G$; \;
        \ForEach{$w \in V(G)$ in the reverse order of $\pi$ }{
        	$\nbr^+(w) \gets \{v|v \in \nbr(w,G) \wedge \pi(v) > \pi(w)\}$; \;
        	$//$ \reflem{sdcheck}\;
        	\ForAll{pairs of $u,v \in \nbr^+(w)$}{
        		\If{$\phi(w,v) + \phi(v,u) < \phi(w,u)$}{ 
        		    delete edge $(w,u)$ from $G'$;\;
        			$\phi(w,u) \gets \phi(w,v) + \phi(v,u)$; \;
        		}
        	}
        }
        \ForEach{$w \in G'$}{
        	$\ev(w) \gets \nbr(w, G')$; \;
        }
\end{algorithm} 


%\begin{algorithm}[htb]
%        \caption{Essential Vertex Sets Generation}
%        \label{alg:evgen}
%        \DontPrintSemicolon
%        \KwInput{A road network $G$}
%        \KwOutput{Essential vertex sets and a \sdg $G''$}
%        $G', G'' \gets$ LD-Graph generated from \refalg{vsgen};\;
%        \ForEach{$w \in V(G')$ in the reverse order of $\pi$ }{
%        	$\nbr^+(w) \gets \{v|v \in \nbr'(w,G') \sqcap \pi(v) > \pi(w)\}$; \;
%        	$//$ \reflem{sdcheck}\;
%        	\ForAll{pairs of $u,v \in \nbr^+(w)$}{
%        		\If{$\phi'(w,v) + \phi'(v,u) < \phi'(w,u)$}{ 
%        		    delete edge $(w,u)$ from $G''$;\;
%        			$\phi'(w,u) \gets \phi'(w,v) + \phi'(v,u)$; \;
%        		}
%        	}
%        }
%        \ForEach{$w \in G''$}{
%        	$\ev(w) \gets \nbr''(w)$; \;
%        }
%\end{algorithm} 

\begin{figure}
    \centering
    \includegraphics[width=0.80\linewidth]{fig1/EPG.pdf}
    \vspace{-0.2cm}
    \caption{\sdg of $G$}
    \label{fig:sdg}
\end{figure}

\stitle{Essential Vertex sets and \sdg Generation.} After achieving \ldg $G'$ and a vertex rank $\pi(\cdot)$ in \refalg{vsgen} in Line 1, in the reverse order of $\pi$ (Line 2), we check the weight of edge to filter the edge $(w,u)$ whose $\phi'(w,u) \neq \sd(w,u)$. Since the shortest distance between any two vertices $u,v$ in $G$ or $G'$ is equal, we denote their shortest distance as $\sd(w,u)$. According to \reflem{sdcheck}, after achieving $nbr^+$ (Line 3), we start to check procedure (Lines 4-8). According to \refalg{evgen}, $G''$ only preserves the edges whose weight is equal to shortest distance between their endpoints in \ldg $G'$. For the clearness of presentation, $G''$ is the \stitle{SD-Graph} of $G$. Based on \refdef{ev}, for each vertex $u \in V(G'')$, $\nbr(u, G'') = \ev(u)$.

%For the clearness of presentation, we call $G''$ as \underline{S}hortest \underline{D}istance Preserved Graph \stitle{(SD-Graph)}, and denote it as $G_{SD}$. Based on \refdef{ev}, for each vertex $u \in G_{SD}$, $\nbr(u, G_{SD}) = \ev(u)$.

\begin{theorem}
	\label{thm:sdg}
	\textbf{Time Complexity Analysis.} The time complexity of \sdg construction is bounded by $O(n \cdot (f^2 + log(n)))$. Here, $f = max_{w \in G}|\keyU(w)|$.
\end{theorem}

\proofsketch
	\refalg{evgen} is bounded by $O(n \cdot (f^2 + log(n)))$ in line 1. In \refalg{vsgen}, each vertex in the graph will be scanned in lines 2-8. Line 3 needs $O(f)$ to the vertex with smallest degree by binary search. Checking edges costs $O(f^2)$ (Lines 5-8). In the lines 12-13, we scan each vertex in the graph to achieve $EV(\cdot)$ bounded by $n \cdot f$. For the edge weight checking part and essential vertex sets generation part (lines 2-8), the time complexity can be bounded by $O(n \cdot(f^2 + log(n)))$. Overall, the time complexity is $O(n \cdot(f^2 + log(n)))$.
\eop


%\begin{example}
%	As shown in \reffig{sdg}, this graph is SD-Graph of the road network in \reffig{roadnetwork}. Take $v_{17}$ as an example, $EV(v_{17}) = \{ v_5, v_{12}, v_{15}, v_{16}, v_{18}, v_{19} \}$, $\keyL(v_{17}) = \{ v_5, v_{12}, v_{15}, v_{16} \}$.
%\end{example}


\begin{example} 
	\ldg $G'$ of the original road network $G$ is shown in \reffig{PG}, the rank $\pi(\cdot)$ is $\{ v_1, v_2,..., v_{20} \}$. We check in the reverse order of $\pi(\cdot)$. %First, we check $v_{20}$. Since $nbr^+(v_{20}) = \emptyset$, we continue to check $v_{19}$. 
	
	We take the procedure details of checking $v_{17}$ and $v_{15}$ as examples in \reffig{check1}. As shown in \reffig{CH_17}, $nbr^+(v_{17}) = \{ v_{18}, v_{19}, v_{20} \}$, since $\phi'(v_{17},v_{19}) + \phi'(v_{19},v_{20}) = 5 + 3 < \phi'(v_{17},v_{20}) = 9$, we delete the edge in $G''$. Simultaneously, we update $8$ to $\phi'(v_{17},v_{20})$ in $G'$, which is used to help weight check for other edges. Since other edges connected to $v_{17}$ satisfy our condition in \reflem{sdcheck}, we keep them in $G''$ and stay their weight in $G'$. 
	%We take the procedure details of checking $v_{15}$ and $v_{10}$ as examples in \reffig{check}. As shown in \reffig{CH_15}, $nbr^+(v_{15}) = \{ v_{16}, v_{17}, v_{20} \}$, since $\phi'(v_{15},v_{16}) + \phi'(v_{16},v_{20}) = 2 + 4 < \phi'(v_{15},v_{20}) = 9$, we delete the edge $(v_{15},v_{20})$ in $G''$. Simultaneously, we update $6$ to $\phi'(v_{17},v_{20})$ in $G'$, which is used to help weight check for other edges. Since other edges connected to $v_{15}$ satisfy our condition in \reflem{sdcheck}, we keep them in $G''$ and stay their weight in $G'$. 
	
	Next, we take the check procedure of $v_{10}$ as an example to illustrate how deleted edges in $G''$ help eight check for other edges. In \reffig{CH_10}, $nbr^+(v_{10}) = \{ v_{14}, v_{15} \}$, since $\phi'(v_{10},v_{14}) + \phi'(v_{14},v_{15}) = 1 + 3 < \phi'(v_{10},v_{15}) = 5$, we delete the edge $(v_{10},v_{15})$ in $G''$. Simultaneously, we update $4$ to $\phi'(v_{10},v_{15})$ in $G'$. Here, we notice the edge $(v_{14}, v_{15})$ is deleted in $G''$. Since $\phi'(v_{14}, v_{15}) = 6$ in \ldg \reffig{PG}, $\phi'(v_{14},v_{16}) + \phi'(v_{16},v_{15}) = 1 + 2 < \phi'(v_{10},v_{15}) = 6$, so the weight is updated as $3$. Without this update, the weight of edge $v_{10},v_{15}$ cannot be checked correctly. So this is why we update the weight of edges in $G'$ in Line 8 of \refalg{evgen}.  
		
	After processing all vertices, \sdg $G''$ is achieved, shown in \reffig{sdg}. Take $v_{17}$ as an example, $EV(v_{17}) = \{ v_5, v_{12}, v_{15}, v_{16}, v_{18}, v_{19} \}$. %$\keyL(v_{17}) = \{ v_5, v_{12}, v_{15}, v_{16} \}$.
\end{example}

% at least one |EU(u)| >= 1 lemma = 连通性不变

\begin{lemma}
	\label{lem:sdc} 
	%Given a road network $G$, \sdg $G_{SD}$ is a \ldg $G_{LD}$ of $G$. $G_{SD} \sqsubseteq G_{LD} \sqsubseteq G$, namely, for each pair of vertices $u,v$ in $G$, we have: $\sd_{G_{SD}}(u,v) = \sd_{G_{LD}}(u,v) = \sd_{G}(u,v)$.
	Given a road network $G$, if for each pair of vertices $u,v$ in $G$ with $\sd_{G_{SD}}(u,v) = \sd_{G}(u,v)$, we call $G_{SD}$ as the \sdg of $G$, denoted as $G_{SD} \sqsubseteq G$.
\end{lemma}

\proofsketch
	Consider the shortest path between any pairs of vertices $v_1,v_n$ in $G$, $\spath(v_1,v_n) = \{ v_1, v_2,..., v_n \}$, the basic distance computation equation for this shortest path is to add the weight of all edges in this path, $\sd(u,v) = \sum_{i \in [1, n-1]} \phi_G(v_i, v_{i+1})$. This equation denotes that the weight of each edge $(v_1, v_{i+1})$ in this shortest path is equal to its shortest distance, namely, $\phi(v_1, v_{i+1}) = \sd(v_1,v_{i+1})$ for $\forall i \in [1, n-1]$. Following \refdef{sdg}, in $G_{SD}$, for $\forall (u,v) \in E(G_{SD})$, $\sd(u,v) = \phi(u,v)$, so $G_{SD}$ does not destroy any shortest paths in $G$. %As \refdef{sdg} shown, \sdg maintain all edges whose weight is equal to the shortest distance in \ldg $G_{LD}$. Since $V(G_{LD}) = V(G) \wedge E(G) \subseteq E(G_{LD})$ and $G_{SD}$ does not destroy shortest path in $G_{LG}$, $G_{SD}$ does not damage the shortest path between each pair of vertices in $G$. 
\eop

\subsection{UG-based \knnindex Construction}
\label{sec:ug}

%Next, we will introduce how to use \sdg and essential vertex sets $EV(\cdot)$ to collect \knnindexcnt. Recall that \sdg maintains all original and new added edges with shortest distance, new added edges $(u,v)$ denotes that there exist a \vspath($u,v$), which is also a \spath($u,v$) such that $\vsd(u,v) = \sd(u,v)$. For any vertex $u$, $\nbr(u)$ in the \sdg contains the original neighbors, partial rank-lower neighbors of $u$ and partial rank-higher neighbors of $u$ in its \sdg. In other words, for all pairs of vertices $u, v$ with $\pi(v) < \pi(u)$ in $G$, only if there is a shortest valley path is also shortest path between $u$ and $v$, there will be an edge in \sdg. If we want to achieve our \knnindex in one-step just like the thought of the naive construction method in \refsec{mi}, this will be unavoidable to cause distance re-use rate low. Since our \sdg already has completed the most important part in \refeq{sdcomp}, essential vertex sets generation $EV(\cdot)$ and the shortest distance computation between vertex and each vertex in its essential vertex set $\sd(u,w), w \in EV(u)$ for $\forall u \in V$. To re-use computed shortest distance sufficiently, we adopt a partial-then-complete index construction strategy. Just constructing partial knn index for $u$ firstly, which only contains vertices with lower ranks than $u$, then we complete \knnindex construction. Before construct the partial knn index, we introduce following definitions:

Next, we will introduce how to use \sdg and essential vertex sets $EV(\cdot)$ to collect \knnindexcnt. Since our \sdg already has completed the important part in \refeq{sdcomp}, essential vertex sets generation $EV(\cdot)$ and the shortest distance computation between vertex and each vertex in its essential vertex set $\sd(u,w), w \in EV(u)$ for $\forall u \in V$. To re-use computed shortest distance sufficiently, we adopt a partial-then-complete index construction strategy. Just constructing partial knn index for $u$ firstly, which only contains vertices with lower ranks than $u$, then we complete \knnindex construction. Before construct the partial knn index, we introduce following definitions:


\begin{definition}
	\label{def:lg}
	\textbf{($u$ Lower Graph)} Given a graph $G$ and its \sdg $G'$, for a vertex $u$, we conduct BFS to explore vertices with lower rank than current explored vertices recursively, until there is no vertex with lower rank than the current explored vertex. In this procedure of BFS, all explored vertices and edges compose to the lower graph for $u$, denoted as $LG(u)$. %Definitely, $UG(u)$ a subgraph of $G'$.
\end{definition}

\begin{example}
	Given a \sdg in \reffig{sdg}, for vertex $v_8$, when exploring from $v_8$ via reaching vertices with lower ranks, each exploring step only explores vertices with lower ranks than the current explored vertex. We conduct BFS to achieve next layer lower vertices $v_2$ and $v_6$, finally, we arrive at $v_{1}$. Since no any vertices have lower ranks than $v_{1}$, we stop the exploring procedure. The lower graph for $v_8$, $LG(v_8)$, is obtained, shown in \reffig{LG_V8}. Similarly, we can achieve $LG(v_{18})$, shown in \reffig{LG_V18}.
\end{example}

\begin{figure}[htb]
 \vspace{-0.5cm}
  \centering
   \subfigcapskip=0pt
   \subfigcaptopadj=0pt
   \subfigure[$LG(v_8)$]
   	 { \includegraphics[width=0.23\linewidth]{fig1/LG8.pdf}
       \label{fig:LG_V8}}
 \subfigure[$LG(v_{18})$]{ \includegraphics[width=0.45\linewidth]{fig1/LG18.pdf}
 	   \label{fig:LG_V18}}
  \vspace{-0.1cm}
 \caption{Lower Graph $LG(v_8)$ and $LG(v_{18})$}
  \label{fig:lg}
\end{figure}

\begin{definition}
	\label{def:pknn}
	%(\stitle{u PKNN}) For each vertex $v$, $v \in \knnalg(u)$, and if $\exists w \in \spath(u,v)$, $w \in \keyL(u)$ ($\spath(u,v) = \vspath(u,v)$), we add all $v$ satisfying above conditions to a set. We define this set as $u$'s \underline{P}artial \underline{T}op-\underline{K} \underline{N}earest \underline{N}eighbors (\pknn), denoted as $\pknnalg(u)$. Namely, $\forall v \in \knnalg(u)$, $\exists w \in \spath(u,v) \wedge w \in \keyL(u)$ $\Rightarrow$ $v \in \pknnalg(u)$.
	%(\stitle{u PKNN}) For each vertex $v$, $v \in \knnalg(u)$, and if $\exists w \in \spath(u,v)$, $w \in \keyL(u)$ ($\spath(u,v) = \vspath(u,v)$), we add all $v$ satisfying above conditions to a set. We define this set as $u$'s \underline{P}artial \underline{T}op-\underline{K} \underline{N}earest \underline{N}eighbors (\pknn), denoted as $\pknnalg(u)$. Namely, $\forall v \in \knnalg(u)$, $\exists w \in \spath(u,v) \wedge w \in \keyL(u)$ $\Rightarrow$ $v \in \pknnalg(u)$.
	%(\stitle{u PKNN}) For each vertex $v$, we save  we add all $v$ satisfying above conditions to a set. We define this set as $u$'s \underline{P}artial \underline{T}op-\underline{K} \underline{N}earest \underline{N}eighbors (\pknn), denoted as $\pknnalg(u)$. 
	%\textbf{($u$ PKNN)} Given a \sdg $G'$ of a graph $G$ and a set of candidate vertices $M$, the \underline{P}artial top-\underline{K} \underline{N}earest \underline{N}eighbors (\pknn), denoted as $\pknnalg(u)$ of a vertex $u$, is the top-K rank-lower nearest neighbors of $u$ with shortest valley distance in $G$ where the set of candidate vertices is $M_u = \{M \cap \{u\} \} \cup_{w \in \keyL(u)} \pknnalg(w)$.
	\textbf{($u$ PKNN)} Given a \sdg $G'$ of a graph $G$, and a set of candidate objects $M$, for each vertex $u \in G$, we pre-achieve its lower graph $LG(u)$, $K$ nearest neighbors of $u$ in its $LG(u)$ is defined as \underline{P}artial top-\underline{K} \underline{N}earest \underline{N}eighbors (\pknn). For $\pknnalg(u)$ of a vertex $u$, its candidate vertex set is $M_u = \{M \cap V(LG(u)) \}$.
	\end{definition}

According to \refdef{pknn}, for the vertex $u$, the distance between $u$ and each vertex $v \in V(LG(u))$ is achieved. Then, it is easy to obtain k nearest neighbors for $u$ after sorting those distances. However, computing these distance is time-consuming. According to \refdef{lg}, we know that each vertex $v \in V(LG(u))$ has a lower rank than $u$. Also, if $v \in \pknnalg(u)$, the path between $u$ and $v$ must pass through $u$'s neighbors in $LG(u)$, then we can further narrow down the computation scope. Before introducing our observations, we first introduce below definitions:
 
\begin{definition}
    \textbf{($u$ Essential Lower Vertex Set)}
	\label{def:el}
	Given a \sdg $G$ and an essential vertex set $EV(u)$ for a vertex $u$, a set of vertices $\keyL(u) = \{ v \in EV(u) | \pi(v) < \pi(u) \}$ is an essential lower vertex cut for $u$ .
\end{definition}

\begin{definition}
	\textbf{(Peak Path)} A path $p(v_1,v_n) = ( v_1,v_2,...,v_n )$ is a peak path, if $\pi(v_1) < \pi(v_2) <...< \pi(v_n)$; that is, the rank of each vertex is higher in the direction from the first vertex $v_1$ to the last vertex $v_n$, denoted as $\ppath(v_1,v_n)$.
\end{definition}

We denote the peak path with smallest distance between $u$ and $v$ as \textbf{\pspath$(u,v)$}, also called as shortest peak path between $u$ and $v$. And we denote the distance of \pspath$(u,v)$ as \textbf{$\psd(u,v)$}, shortest peak distance.

\begin{example}
	In the lower graph of $v_8$, $LG(v_8)$, shown in \reffig{LG_V8}, $P_1 = (v_1, v_2, v_6, v_8)$ is a peak path between $v_1$ and $v_8$. $P_2 = (v_1, v_2, v_8)$ is a peak path between $v_1$ and $v_8$. $P_2$ is the shortest peak path between $v_1$ and $v_8$, since distance of $\pspath(v_1,v_8)$ is smallest. The shortest peak distance between $v_1$ and $v_8$ is $4$, namely, $\psd(v_1,v_8) = 4$.
\end{example}

%minimize computational cost = maximize distance reuse rate + reduce unnecessary computation + explore 

\begin{lemma}
	\label{lem:first}
	Given a \sdg of the graph $G$ and the vertex with the lowest rank $u_1$, $\pknnalg(u_1) = \{M \cap \{ u_1 \}\}$.  
\end{lemma} 

\proofsketch
	According to \refdef{lg}, we can know the lower graph of the vertex with lowest vertex $LG(u_1)$ only contain itself. Based on \refdef{pknn}, $\pknnalg(u_1) = \{M \cap \{ u_1 \}\}$.
\eop


\begin{lemma}
	\label{lem:pknn}
	Given a \sdg of the graph $G$, $\pknnalg(u) \subseteq \{M \cap \{ u \}\} \cup_{w \in \keyL(u)} \pknnalg(w)$.  
\end{lemma} 

\proofsketch
	Following \refdef{pknn}, \pspath($u,v$) must pass through at least one vertex $w \in \keyL(u)$, which also means that for $\forall v \in \pknnalg(u)$, $v$ must belong to $\pknnalg(w)$ for at least one $w \in \keyL(u)$. We prove the lemma by contradiction. We assume that there exists a vertex $v \in \pknnalg(u)$, but $v \notin \cup_{w \in \keyL(u)} \pknnalg(w)$. There exists one $w \in \keyL(u)$ such that for $\forall v_i \in \pknnalg(w)$, $1 \leq i \leq k$, we have $\psd(w,v_i) < \psd(w,v)$. Then $\phi'(u, w) + \psd(w,v_i) < \phi'(u,w) + \psd(w,v)$. It means there are at least $k$ vertices whose distance to $u$ is smaller than the shortest peak distance between $u$ and $v$, which contradicts $v \in \pknnalg(u)$. The proof completes.
\eop

\begin{lemma}
	\label{lem:pknnDist}
	Given a \sdg $G'$ of the graph $G$, $\forall v \in \pknnalg(u)$, $\psd(u,v) = min_{ w \in \keyL(u)} \{ \phi'(u,w) + \psd(w,v) \}$.  
\end{lemma} 

\proofsketch
	According to the definition of valley path, we can know that for each vertex $u$ in $G$, the valley paths between any other vertex $v$ with lower rank than $u$ in $G$ and $u$ must pass through at least one vertex $w \in \keyL(u)$. Similarly, for $u$ and $v$, \pspath($u,v$) must pass through at least one vertex $w \in \keyL(u)$. So we have $\psd(u,v) = min_{ w \in \keyL(u)} \{ \phi_{G'}(u,w) + \psd(w,v) \}$.
\eop

Based on \reflem{first} and \reflem{pknn}, we adopt a low-to-up(LTU) direction to construct \pknnindex to make full use of computed distance via \reflem{pknnDist} and narrow down the computation scope via \reflem{pknn}. The \pknnindex construction is shown in \refalg{naivecon}

\begin{lemma}
	\label{lem:ral_p_v}
	Given a \sdg of the graph $G$, $\forall v \in \knnalg(u)$ s.t. $\pi(v) < \pi(u)$, $\exists w \in \spath(u,v)$ s.t. $w \in \keyL(u)$ $\Rightarrow$ $v \in \pknnalg(u)$.
\end{lemma}

\proofsketch
	If $v \in \knnalg(u) \wedge \pi(v) < \pi(u)$ and $\exists w \in \spath(u,v)$ s.t. $w \in \keyL(u)$, we can achieve $\psd(u,v) = \sd(u,v)$. We prove the lemma by contradiction. We assume that there exists a vertex $v$ satisfying above condition, but $v \notin \pknnalg(u)$. $v \notin \pknnalg(u)$ denotes that there are at least k vertices ($v_i, i \in [1, k]$) whose shortest valley distance is smaller than $\psd(u,v)$, namely $\psd(u,v_i) < \psd(u,v), i \in [1, k]$. According to the relationship between shortest distance and shortest valley distance, $\sd(u,v) \leq \psd(u,v)$. Since $\sd(u,v_i) \leq \psd(u,v_i) < \psd(u,v), i \in [1, k]$, there are at least k vertices who shortest distance with $u$ is smaller than $\sd(u,v)$. then we conclude that $v \notin \knnalg(u)$, which contradicts the assumption. So the assumption is not valid. Our proof completes.
\eop

\begin{lemma}
	\label{lem:ral_p_v_rev}
	Given a \sdg of the graph $G$, $v \in \pknnalg(u)$ s.t. $v \in \knnalg(u)$ and $\exists w \in \spath(u,v)$ s.t. $w \in \keyL(u)$ $\Rightarrow$ There exist a shortest peak path between $u$ and $v$ which also is a shortest path. % $\pspath(u,v)$ $\spath(u,v)$.
\end{lemma}

\proofsketch
	$v \in \pknnalg(u)$ denotes that $\pi(v) < \pi(u)$, also \pspath($u,v$) must pass through at least one vertex $w \in \keyL(u)$. When \pspath($u,v$) pass through several vertices, we choose the vertex with highest rank as $w$. Following this step, we continue to explore next $w'$ until we meet $v$. Following \refdef{lg} and \refdef{sdg}, all shortest valley paths are converted into edges into original graph, so there must be at least one $\spath(u,v)$ is a shortest peak path.
\eop


\begin{figure}
    \centering
    \includegraphics[width=0.80\linewidth]{fig1/PKNN_C.pdf}
    \vspace{-0.2cm}
    \caption{$\pknnalg(v_{17})$ Construction}
    \label{fig:PKNN_N}
\end{figure}

%\begin{figure}
   % \centering
    %\includegraphics[width=0.80\linewidth]{fig1/PKNN_CNN.pdf}
   % \vspace{-0.2cm}
  %  \caption{$\pknnalg(v_{17})$ Construction}
 %   \label{fig:PKNN_N}
%\end{figure}


%\begin{figure}
%    \centering
%    \includegraphics[width=0.80\linewidth]{fig1/PKNN_CN.pdf}
%    \vspace{-0.2cm}
%    \caption{$\knnalg(v_{17})$  Construction}
%    \label{fig:PKNN_N}
%\end{figure}

Since $\pknnalg(w)$ contains top-k nearest neighbors passing through $\keyL(u)$, only the vertices $v \in \knnalg(u)$ passing through $\keyU(u)$ do not be explored. Since only partial KNN $\pknnalg(p)$ for $\forall p \in \keyU$ is achieved, if we explore $\cup_{p \in \keyU(u)} \pknnalg(p)$, we only grab the vertices with non-higher ranks than each $p$, while the vertices with higher ranks than each $p$ will be missed. Therefore, we have to continue to explore vertices via $\keyL(u)$ iteratively until all higher-rank vertices are explored. Next, we will introduce the upper graph definition to support \knnindex construction for each vertex:
% the vertices, whose shortest path between vertices and $u$ passes through rank higher vertices, will be missed.

\begin{definition}
	\label{def:ug}
	\textbf{($u$ Upper Graph)} Given a graph $G$ and its \sdg $G'$, for a vertex $u$, we conduct BFS to explore vertices with higher rank than current explored vertices recursively, until there is no vertex with higher rank than the current explored vertex. In this procedure of BFS, all explored vertices and edges compose to the upper graph for $u$, denoted as $UG(u)$. %Definitely, $UG(u)$ a subgraph of $G'$.
\end{definition}

\begin{example}
	Given a \sdg in \reffig{sdg}, for vertex $v_1$, when exploring from $v_1$ via reaching vertices with higher ranks, each exploring step only explores vertices with higher ranks than the current explored vertex. We conduct BFS to achieve next layer higher vertices $v_2$ and $v_6$, then probe $v_7$ and $v_8$, finally, we arrive at $v_{20}$. Since no any vertices have higher ranks than $v_{20}$, we stop the exploring procedure. The upper graph for $v_1$, $UG(v_1)$, is obtained, shown in \reffig{UG_V1}. Similarly, we can achieve $UG(v_{16})$, shown in \reffig{UG_V16}.
\end{example}


\begin{figure}[htb]
 \vspace{-0.1cm}
  \centering
   \subfigcapskip=0pt
   \subfigcaptopadj=0pt
   \subfigure[$UG(v_1)$]
   	 { \includegraphics[width=0.37\linewidth]{fig1/UG_V1N.pdf}
       \label{fig:UG_V1}}
 \subfigure[$UG(v_{16})$]{ \includegraphics[width=0.442\linewidth]{fig1/UG_V16N.pdf}
 	   \label{fig:UG_V16}
	 }
  \vspace{-0.1cm}
 \caption{Upper Graph $UG(v_1)$ and $UG(v_{16})$}
  \label{fig:ug}
\end{figure}

\begin{lemma}
	\label{lem:ugsize}
	Given a \sdg $G'$ of a road network $G$, the number of vertices in the upper graph for each vertex $u \in V(G')$ is bounded by $l$, namely, $|V(UG(u))| \leq l$. In practice, the size of upper graph is far less than the number of vertices in the whole graph $G$, namely, $l \ll n$.
\end{lemma}

\proofsketch

\eop

After \pknnindex construction, we directly achieve the \knn for each vertex via Forward-Dijkstra. Forward-Dijkstra only explores vertices with higher rank than current explored vertices, namely, Forward-Dijkstra for $u$ is just exploring vertices along its upper graph $UG(u)$.

\begin{lemma}
	\label{lem:naiveknn}
	%Given a \sdg of the graph $G$, 
	$\knnalg(u) \subseteq \pknnalg(u) \cup_{w \in V(UG(u))} \pknnalg(w)$.
\end{lemma}

\proofsketch
	According to \refpro{vcknn}, this lemma is easy to be proved.
\eop


\begin{lemma}
	\label{lem:naiveknnDist}
	%Given a \sdg of the graph $G$, 
	$\forall v \in \knnalg(u), \sd(u,v) = min_{w \in V(UG(u))} \{ \sd(u,w) + \psd(w,v) \}$.
\end{lemma}

\proofsketch
	Based on \reflem{naiveknn}, for $\forall v \in \knnalg(u)$, $v$ comes from $\pknnalg(u) \cup_{w \in UG(u)} \pknnalg(w)$, so $\psd(w,v)$ can be directly achieved. Recall \refpro{sd} and \reflem{ral_p_v}, this step only needs to grab the vertices $v$ such that $\exists w \in \spath(u,v) \wedge w \in \keyU(u)$. For each $v \in \knnalg(u)$ satisfying the above condition, \spath($u,v$) must pass through one vertex $w \in \keyU(u)$. So $\sd(u,v) = \sd(u,w) + \sd(w,v)$. $\sd(u,w)$ is calculated in Forward-Dijkstra in Line 12 of \refalg{naivecon}. For $\sd(w,v)$ computation, there is several cases here: (1) When $\spath(w,v)$ is a valley path, $\sd(w,v) = \vsd(w,v)$, which can be from $\pknnalg(w)$ directly. (2) $\spath(w,v)$ is not a peak path, we aim to find the vertex $p$ with highest rank in $\spath(w,v)$. According to \refdef{ug}, $p$ must exists in $UG(u)$. Here, $\sd(u,v)$ also can be calculated as $\sd(u,v) = \sd(u,p) + \sd(p,v)$. $\sd(u,m)$ has been calculated in Forward-Dijkstra in Line 12 of \refalg{naivecon}. For $\sd(p,v)$, $\spath(p,v)$ is definitely a valley path, $\sd(p,v) = \psd(p,v)$, which can be from $\pknnalg(p)$ directly.  
\eop

\textbf{UG \knnindex Construction.} Line 1 uses \refalg{evgen} to generate a \sdg $G'$ of the input road network $G$, Line 2 achieves $\pknnalg(\cdot)$ using the \pknnindex generation part of \refalg{naivecon}. Based on \reflem{finalv}, to maximize distance re-use rate, we adapt a up-to-low direction to construct $\knnalg(\cdot)$. We initialize $\mathbb{U}$ as $\emptyset$ and $\knnalg(\cdot)$ as $\emptyset$ for each vertex in $G$. In the reverse order of the vertex rank $\pi(\cdot)$ (Line 4), we first get a small candidate set $\mathbb{U}$ for $u_i$ based on \reflem{knn} in Line 5. Following \reflem{knnDist}, we calculate the distance between $u_i$ and each vertex $v$ in the candidate set $\mathbb{U}$ (Lines 6-9). We sort the vertices in $\mathbb{U}$ in the ascending distance order (Line 10). Then, we grab $k$ vertices with smallest distance to $u$ as $\knnalg(u)$.

\begin{theorem}
	\label{thm:naiveknn} 
	\textbf{Time Complexity Analysis.} The time complexity of UG \knnindex construction is bounded by $O(n \cdot (f^2 + log(n)+ f \cdot l \cdot log(l)) + (f+l) \cdot k)$ ($f = max_{v \in V}|\keyU(v)|$).	
\end{theorem}


\proofsketch
	Referring to \refthm{ldg}, the time complexity of vertex set and \ldg generation is $O(n \cdot (f^2 + log(n)))$ (line 1). Line 4 can be bounded by $O(f \cdot k)$, since each vertex $u$ is only explored by its $\keyU(u)$, which completes in $O(f)$ time, and the size of \pknnindex for $u$ can be bounded by $O(k)$. For \pknnindex construction part (lines 3-8), the time complexity can be bounded by $O(n \cdot f \cdot k)$. For the \knn index construction (lines 9-16), referring to \reflem{ugsize}, line 11 can be bounded by $O(l \cdot k)$. Constructing $UG(u_i)$ by BFS (line 10) and computing $\sd(u_i, \cdot)$ by \kw{Dijkstra's} algorithm (line 12) cost $O(f \cdot l \cdot log(l))$ time. For the distance computation in lines 13-14, since $\pknnalg(w)$ stores all shortest peak distance between $w$ and $v$ for $\forall v \in \pknnalg(w)$, $\psd(w,v)$ can be obtained in $O(1)$ time. During the time of obtaining $\mathbb{U}$, the distance computation can be calculated directly. Overall, the UG-Based \knnindex construction costs $O(n \cdot (f^2 + log(n) + f \cdot l \cdot log(l)) + (f+l) \cdot k)$.
	%Referring to \reflem{knn}, for $\forall v \in \knnalg(u)$, we know that $v$ comes from $\cup_{w \in \keyU(u)} \knnalg(w)$, so that $\sd(w,v)$ can be achieved directly from $\knnalg(w)$ in $O(1)$.
\eop

In the following, we provide an example to illustrate \refalg{naivecon}:

\begin{example}
	\label{ex:ugcon}
	\reffig{sdg} is the \sdg of the original graph in \reffig{roadnetwork}. We take $\knnalgex(v_{17})$ construction as an example. In \reffig{sdg}, according to \refdef{el}, we can obtain $\keyL(v_{17}) = \{ v_5, v_{12}, v_{15}, v_{16} \}$. $\pknnalgex(v_{5}) = \{v_{5} | 0 \}$, $\pknnalgex(v_{12}) = \{ v_{12}, v_{5}, v_{11}, v_{4}, v_{3} | 0, 1, 1, 2, 3\}$, $\pknnalgex(v_{15}) = \{v_{15} | 0 \}$, $\pknnalgex(v_{16}) = \{v_{16}, v_{14}, v_{10}, v_{15} | 0, 1, 2, 2 \}$. Based on \reflem{naiveknn} and \reflem{naiveknnDist}, the small candidate set $\mathbb{C}$ with shortest peak distance for $\pknnalgex(v_{17})$ is achieved, $\mathbb{C} = \{ \mathbb{M} \cap \{ v_{17} \} \} \cup_{ w \in \keyL(v_{17}) } \pknnalgex(w) = \{ v_{17}, v_{5}, v_{12}, v_{15}, v_{11}, v_{4}, v_{16}, v_{3}, v_{14}, v_{10} | 0, 2, 3, 3, 4, 5, 5, 6, 6, 7 \}$. Sorting the distance, $\pknnalgex(v_{17}) = \{ (v_{17},0), (v_{5},2), (v_{12},3), (v_{15},3), (v_{11},4) \}$.
	
	According to \refdef{ug}, $UG(v_{17})$ is shown in \reffig{UG_V17}, $V(UG(v_{17})) = \{ v_{17}, v_{18}, v_{19}, v_{20} \}$. Following \reflem{naiveknn}, we first achieve $\pknnalgex(v_{18}) = \{ (v_{18},0), (v_{11},2), (v_{13},3), (v_{12},3), (v_{5},4) \}$, $\pknnalgex(v_{19}) \\= \{ (v_{19},0), (v_{11},1), (v_{9},2), (v_{12},2), (v_{5},3) \}$, and $\pknnalgex(v_{20}) = \{ (v_{20},0),\\ (v_{9},1), (v_{7},2), (v_{8},2), (v_{19},3) \}$. According to \reflem{naiveknn}, According to \reflem{naiveknnDist}, we get the small candidate set $\mathbb{U}=\{ v_{17}, v_{5}, v_{12}, v_{15}, \\v_{11}, v_{18}, v_{19}, v_{9}, v_{20}, v_{13}, v_{7}, v_{8} \}$. From $\mathbb{U}$, we select $k$ nearest vertices as $\knnalg(v_{17}) = \{ (v_{17},0), (v_{5},2), (v_{12},3), (v_{15},3), (v_{11},4) \}$. %0,2,3,3,4,5,6,7,8,9,10,10
\end{example}

\begin{figure}[htb]
 \vspace{-0.1cm}
  \centering
   \subfigcapskip=0pt
   \subfigcaptopadj=0pt
   \subfigure[$UG(v_{17})$]
   	 { \includegraphics[width=0.3\linewidth]{fig1/UG_V17.pdf}
       \label{fig:UG_V17}}
 \subfigure[UG Construction for $\knnalg(v_{17})$]{ \includegraphics[width=0.7\linewidth]{fig1/PKNN_Naive.pdf}
 	   \label{fig:NaiveCon}
	 }
  \vspace{-0.1cm}
 \caption{UG $\knnalg(v_{17})$ Construction}
  \label{fig:pknn_naive}
\end{figure}



\begin{algorithm}[htb]
    \caption{UG \knnindex construction}
    \label{alg:naivecon}
    \DontPrintSemicolon
        \KwInput{A Road Network $G$}
        \KwOutput{\knnindex}
        $G' \gets$ \sdg generated from \refalg{evgen}; \;
        $\mathbb{C} \gets \emptyset$, $\mathbb{U} \gets \emptyset$, $\pknnalg(\cdot) \gets \emptyset$, $\knnalg(\cdot) \gets \emptyset$; \; 
        \ForEach{$i = 1,2,...,n$}{
            $\mathbb{C} \gets \{\mathcal{M} \cap \{ u_i \} \} \cup_{w \in \keyL(u_i)} \pknnalg(w)$; $//$ \reflem{pknn} \;
            \ForEach{$v \in \mathbb{C}$}{
            %$ \overline{\sd}(u_i,v) \gets \min_{w \in \keyL(u_i)} \phi_{G'}(u_i,w) + \overline{\sd}(w,v); $ \;
            $ \psd(u_i,v) \gets \min_{w \in \keyL(u_i)} \{ \phi'(u_i,w) + \psd(w,v)\}$; 
            }
            sort vertices in $\mathbb{C}$; \;
            $\pknnalg(u_i) \gets$ top-k nearest vertices in $\mathbb{C}$; \;
        }
        \ForEach{$i = 1,2,...,n$}{
        	Construct $UG(u_i)$ following \refdef{ug}; \;
        	$\mathbb{U} \gets \pknnalg(u_i) \cup_{w \in V(UG(u_i))} \pknnalg(w)$; $//$ \reflem{naiveknn}\;
        	Compute $\sd(u_i,w)$ for each vertex $w$ in $V(UG(u_i))$; \;
        	\ForEach{$v \in \mathbb{U}$}{
            	%$\sd(u_i,v) \gets \min_{w \in UG(u_i)} \sd(u_i,w) + \overline{\sd}(w,v); $ \;
            	$\sd(u_i,v) \gets \min_{w \in UG(u_i)} \sd(u_i,w) + \psd(w,v)$;%\{ \sd(u_i,w) + \psd(w,v) \}$;
            }
        	sort vertices in $\mathbb{U}$; \;
            $\knnalg(u_i) \gets$ top-k nearest vertices in $\mathbb{U}$; \;
        }
\end{algorithm}



%\begin{figure*}[!tb]
%	\centering
%	\subfigcapskip=0pt
%	\subfigure[PKNN Con]{\includegraphics[width=0.35\linewidth]{fig1/PKNN_C.pdf}} \hspace{0.2cm}
%	\subfigure[Upper Graph $UG(V_{17})$]{\includegraphics[width=0.15\linewidth]{fig1/UG_V17.pdf}}
%	     \hspace{0.2cm}
%	\subfigure[Naive KNN Con]{\includegraphics[width=0.35\linewidth]{fig1/PKNN_Naive.pdf}}\\
%	\vspace{-0.3cm}
% \vspace{0.2cm}
%	\caption{Naive Construction}
%	\label{fig:cases}
%	 \vspace{-0.3cm}
%  \end{figure*}



\subsection{UTL \knnindex Construction}
\label{sec:utl}

In this subsection, we show how to further optimize \knnindex in \refalg{naivecon}, we consider two aspects to improve the algorithm. First, for each vertex $u$, we need to construct its upper graph $UG(v)$ and compute the single source shortest distances from $v$ to all other vertices in $UG(v)$, which is costly. We consider how to compute \knnindex without building the lower graph $UG(v)$. Second, the vertex labels are computed individually in \refalg{naivecon}. To save computational cost, we will consider cost sharing when computing the labels for different vertices. Note that the upper graph $UG(v)$ is a supergraph of $UG(u)$ for any $u \in UG(v)$. This means that we can reuse the label information in $UG(u)$ when computing the label for $v$. Also, we have following new observations to make the distance reuse more sufficiently.
%Drawbacks:
%\begin{enumerate}
%	\item Even Forward-Dijkstra is more efficient than original Dijkstra, Forward-Dijkstra is still costly. We consider how to calculate labels without Forward-Dijkstra.
%	\item Above UG \knnindex labels \knnindex for each vertex independently, we consider cost sharing.
%\end{enumerate}


\begin{definition}
    \textbf{($u$ Essential Upper Vertex Set)}
	\label{def:eu}
	Given a \sdg $G$ and an essential vertex set $EV(u)$ for a vertex $u$, a set of vertices $\keyU(u) = \{ v \in EV(u) | rank(v) > rank(u) \}$ is an essential upper vertex cut for $u$ .
\end{definition}

Given a \sdg $G$, for every $ u \in G$, we have $EV(u) = \keyU(u) \cup \keyL(u)$.

\begin{lemma}
	\label{lem:finalv}
	Given a \sdg of the graph $G$, the vertex with the highest rank $u_n$, we have $\pknnalg(u_n) = \knnalg(u_n)$.
\end{lemma}

% 证明 C vdist(u,v) = dist(u,v).
\proofsketch
	Consider the rank generated from \refalg{vsgen}, the vertex with the heighest rank $u_n$, its $EV(u_n) = \keyL(u_n) = \keyU(u_n)$, so $\pknnalg(v_n) = \knnalg(v_n)$. When computing its $\pknnalg(v_n)$, \refalg{naivecon} scans each $w \in \keyL(u_n)$, $\forall v \in \pknnalg(v_n), \psd(u_n,v) = min_{ w \in \keyL(u)} \{ \sd(u_n,w) + \psd(w,v) \}$. Since $EV(u_n) = \keyL(u_n)$, so according to \refpro{sd}, $\sd(u_n,v) = min_{ w \in \keyL(u)} \{ \sd(u_n,w) + \psd(w,v) \}$. Since the shortest distance between all vertices $v$ and $u_n$ is calculated, $\pknnalg(v_n) = \knnalg(v_n)$.
\eop

Based on \reflem{finalv}, to maximize distance re-use and avoid unnecessary vertices exploration, we adopt Up-to-Low (UTL) direction to construction our \knnindex. We will prove our algorithm correctness as following lemmas:

\begin{lemma}
	\label{lem:knn}
	Given a SD-Graph of the graph $G$, for each vertex $u \in G$, its essential upper vertex set $\keyU(u)$, we have:
	 
	\hspace{4em}$\knnalg(u) \subseteq \pknnalg(u) \cup_{w \in \keyU(u)} \knnalg(w)$.
\end{lemma}

\proofsketch
	According to the \refpro{vcknn}, this is easy to be proved.
\eop


\begin{lemma}
	\label{lem:knnDist}
	Given a \sdg of the graph $G$, $\forall v \in \knnalg(u),$ we have:
	
$\sd(u,v) = min \{ min_{w \in \keyU(u)} \{ \sd(u,w) + \sd(w,v) \}, \psd(u,v) \}$. 
\end{lemma}
%\begin{equation}
%	\label{eq:knnDisCom}
%	\sd(u,v) = min \{ min_{w \in \keyU(u)} \{ \sd(u,w) + \sd(w,v) \}, \vsd(u,v) \}.
%\end{equation}

\proofsketch
	According to \refdef{sdg}, the weight of each edge is the shortest distance for the endpoints of the edge, namely $\phi(u,v) = \sd(u,v)$. So for $\forall w \in \keyU(u)$, we have $\phi(u,w) = \sd(u,w)$. Based on \refpro{sd}, we know that the equation in \reflem{knnDist} can calculate the distance for the shortest paths between $v$ and $u$ passing through $w \in \keyU(u)$. Based on \reflem{ral_p_v_rev}, we know when $\psd(u,v)$ is smaller, $\psd(u,v) = \sd(u,v)$. So we can get the shortest distance for each $v$ and $u$ according to the equation in \reflem{knnDist}.
\eop

\textbf{UTL \knnindex Construction.} Line 1 uses \refalg{evgen} to generate a \sdg $G'$ of the input road network $G$, Line 2 achieves $\pknnalg(\cdot)$ using the \pknnindex generation part of \refalg{naivecon}. Based on \reflem{finalv}, to maximize distance re-use rate, we adapt a up-to-low direction to construct $\knnalg(\cdot)$. We initialize $\mathbb{U}$ as $\emptyset$ and $\knnalg(\cdot)$ as $\emptyset$ for each vertex in $G$. In the reverse order of the vertex rank $\pi(\cdot)$ (Line 4), we first get a small candidate set $\mathbb{U}$ for $u_i$ based on \reflem{knn} in Line 5. Following \reflem{knnDist}, we calculate the distance between $u_i$ and each vertex $v$ in the candidate set $\mathbb{U}$ (Lines 6-9). We sort the vertices in $\mathbb{U}$ in the ascending distance order (Line 10). Then, we grab $k$ vertices with smallest distance to $u$ as $\knnalg(u)$.

\begin{theorem}
	\label{thm:tc_utl}
	\textbf{Time Complexity Analysis.} The time complexity of UTL \knnindex construction is bounded by $O(n \cdot (f^2 + logn) + n \cdot f \cdot k)$ ($f = max_{v \in V}|\keyU(v)|$).
\end{theorem}

\proofsketch
	Referring to \refthm{sdg}, the time complexity of essential vertex set  and \sdg generation is $O(n \cdot (f^2 + log(n)))$ (line 1). The maximum size of $\mathbb{U}$ is bounded by $O(f \cdot k)$, so the time complexity (line 5) is $O(f \cdot k)$. The distance calculation (lines 6-9) and candidates selection (line 5) can be done simultaneously. Overall, the time complexity (lines 4-11) is $O(n \cdot f \cdot k)$. So UTL $\knnindex$ construction can be bounded by $O(n \cdot f^2 + n \cdot f \cdot k)$.
\eop



In the following, we provide an example to illustrate \refalg{utl}:

\begin{example}
	We take \knnindex construction for $v_{17}$ as an example in \reffig{knn}. Since UTL construction and UG construction method both own the same procedure of \pknnindex construction, $\pknnalgex(v_{17})$ construction procedure is shown in \refex{ugcon}. Here, we focus on the procedure details of $\knnalgex(v_{17})$ construction. On the \sdg in \reffig{sdg}, $\keyU(v_{17}) = \{ v_{18}, v_{19} \}$. According to \reflem{knn}, we can obtain the small candidate set $\mathbb{U}$ for $v_{17}$ via $\pknnalgex(v_{17}) \cup_{w \in \keyU(v_{17})} \knnalgex(w)$. $\pknnalgex(v_{17}) = \{ (v_{17}, 0), (v_{5}, 2), (v_{5}, 3), (v_{12},\\ 3), (v_{11}, 4) \}$, $\knnalgex(v_{18}) = \{ (v_{18}, 0), (v_{11}, 2), (v_{12}, 3), (v_{13}, 3), (v_{19}, 3) \}$, and $\knnalgex(v_{19}) = \{ (v_{19}, 0), (v_{11}, 1), (v_{12}, 2), (v_{9}, 2), (v_{18}, 3) \}$. After distance computation \reflem{knnDist}, $\mathbb{U} = \{ v_{17}, v_{5}, v_{15}, v_{12}, v_{11}, v_{18}, v_{9}\}$. After sorting in ascending distance order, the final k nearest neighors for $v_{17}$ is $\knnalgex(v_{17}) = \{ (v_{17}, 0), (v_{5}, 2), (v_{15}, 3), (v_{12}, 3), (v_{11}, 4) \}$.
\end{example}


%\begin{figure}
%    \centering
%    \includegraphics[width=0.70\linewidth]{fig1/KNN_CON.pdf}
%    \vspace{-0.2cm}
%    \caption{$\knnalg(v_{17})$  Construction}
    %\vspace{-0.4cm}
%    \label{fig:KNN}
%\end{figure}



%\begin{figure}
%    \centering
%    \includegraphics[width=0.70\linewidth]{fig1/KNN_CN.pdf}
%    \vspace{-0.2cm}
%    \caption{$\knnalg(v_{17})$  Construction}
%    \label{fig:KNN}
%\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=0.80\linewidth]{fig1/KNN_C.pdf}
    \vspace{-0.2cm}
    \caption{$\knnalg(v_{17})$ Construction}
    \label{fig:knn}
\end{figure}


\begin{algorithm}[tb]
    \caption{UTL \knnindex construction}
    \label{alg:utl}
    \DontPrintSemicolon
        \KwInput{A Road Network $G$}
        \KwOutput{\knnindex}
        $G' \gets$ \sdg  generated from \refalg{evgen}; \;
        $\pknnalg(\cdot) \gets$ \pknnindex derived from \refalg{naivecon}; \; 
        $\mathbb{U} \gets \emptyset$, $\knnalg(\cdot) \gets \emptyset$; \; 
        \ForEach{$i = n, n-1,..., 1$}{
        	$\mathbb{U} \gets \pknnalg(u_i) \cup_{w \in \keyU(u_i)} \knnalg(w)$; $//$ \reflem{knn} \;
        	\ForEach{$v \in \mathbb{U}$}{$//$ \reflem{knnDist} \;
        		$\overline{\sd}(u_i,v) \gets  \min_{w \in \keyU(u_i)} \{ \phi'(u_i,w) + \sd(w,v) \};$\;
        		$\sd(u_i,v) \gets min\{\overline{\sd}(u_i,v), \psd(u_i,v)\}$; \;
            }
        	sort vertices in $\mathbb{U}$; \;
            $\knnalg(u_i) \gets$ top-k nearest vertices in $\mathbb{U}$; \;
        }
        return $\knnalg(\cdot)$; \;
\end{algorithm}


\subsection{Candidate Object Updates}
\label{sec:update}
Our index contains \knn for all vertices, however, it is unnecessary to update \knn for the whole vertices only due to several objects insertion or deletion. Since some object updates only work for a small part of query vertices, other queries are not affected by these updates. It is unnecessary to be \stitle{\emph{eager}} to update index for all vertices. We adopt a \stitle{\emph{lazy}} update strategy to update index for vertices which are not queried. Especially, we conduct a partial update strategy, which updates \pknnindex first. For queries after updating, via the updated \pknnindex, we make a specific \knnindex update for the query vertex. %first, and then return the after-updated and exact \knn for other query vertices. %and common updated \knn sharing property

\subsubsection{\pknn Update for Objects Deletion.} The algorithm for deleting a candidate vertex is called \emph{KNN-Delete}, and the pseudocode is shown in \refalg{delete}.

We construct $UG(u)$ for the inserted vertex $u$ in line 1. If $\pknnalg(u_i)$ does not contain $u$, we directly go to the next vertex in $UG(u)$ in lines 3-4. Otherwise, we delete $u$ from $\pknnalg(u_i)$ in line 5. Similar to the \pknnindex construction, we update $\pknnalg(u_i)$ via constructing a candidate set $\mathbb{C}$ from $\cup_{w \in \keyL(u_i)}\pknnalg(w) \setminus \pknnalg(u_i)$ in line 6. When there exists vertices in $\mathbb{C}$, we insert the vertex $v$ with smallest shortest peak distance into the end to $\pknnalg(u_i)$ in lines 7-9. Based on the doubly linked list, we efficiently locate the vertices $u_i$ in line 2 of \refalg{delete}. It takes constant time to check whether a vertex belongs to $\pknnalg$ of the other vertex.


%First, we record the rank $\pi(u)$ of the deleted vertex $u$ in line 1. In line 2, we only consider the vertex $v$ whose $\pknnalg(v)$ contains $u_d$. Similar to the index construction, we update $\pknnalg(u_i)$ via $\pknnalg(w)$ ($w \in \keyL(u_i)$) in line 4. Note that we do not need to recompute  of $\pknnalg(w)$. Let $m$ be the new vertex added to $\pknnalg(u_i)$. The shortest distance from $m$ to $u_i$ must be not smaller than that from any vertex in the existing $\pknnalg(u_i)$ to $u_i$ and not larger than that from any other candidate to $u_i$. Therefore, in lines 5–8, we scan the candidate vertices and derive such vertex $v$. We use a doubly linked list to connect the same vertices in \pknn. Based on the doubly linked list, we efficiently locate the vertices $u_i$ in line 2 of \refalg{delete}. It takes constant time to check whether a vertex belongs to $\pknnalg$ of the other vertex.

\begin{algorithm}[htb]
        \caption{\emph{KNN-Delete}}
        \label{alg:delete}
        \DontPrintSemicolon            
            \KwInput{$\knnalg(\cdot)$ and a deleted vertex $u$}
            \KwOutput{The updated $\pknnalg(\cdot)$}
            $UG(u) \gets$ the upper graph of $u$;\;
            	\For{$i = 1, 2,...,l$ in the positive rank in $UG(u)$ }{
           		\If{$u \notin \pknnalg(u_i)$}{continue;}
           		delete $u$ from $\pknnalg(u_i)$;\;
            		$\mathbb{C} \gets \cup_{w \in \keyL(u_i)} \pknnalg(w) \setminus \pknnalg(u_i)$;\;
            		\If{$\mathbb{C} \neq \emptyset$}{
            			$v \gets argmin_{v \in \mathbb{C}}  \psd(v,u_i)$;\;
            			insert $v$ into the end of $\pknnalg(u_i)$;\;
            		}
            }
\end{algorithm} 


\begin{theorem}
	Given the \knn of a graph $G$ and a deleted candidate vertex $u$, the time complexity of \refalg{delete} is bounded by $O(l \cdot k \cdot p)$, where $p = max_{u \in V} |\keyL(u)|$.
\end{theorem}

\proofsketch
	According to \reflem{ugsize}, the size of upper graph for $u$ is bounded by $l$. In line 5, the size of $\mathbb{C}$ is $|\keyL(u_i)| \cdot k \leq p \cdot k$. Therefore, the total time complexity of \refalg{delete} is $O(l \cdot p \cdot k)$.
\eop

The first part $O(l)$ in the time complexity can be very small practically, since we only process the vertex $u_i$ such that $u \in \pknnalg(u_i)$.

\subsubsection{Special Query after deleting objects} The algorithm for KNN query for $v$ after deleting a candidate vertex $u$ is shown in \refalg{delete_tar}.

We construct $UG(v)$ for the query vertex $v$ in line 1. If $\pknnalg(u_i)$ does not contain $u$, we directly go to the next vertex in $UG(v)$ in lines 3-4. Otherwise, we delete $u$ from $\pknnalg(u_i)$ in line 5. Similar to the \knnindex construction, we update $\knnalg(u_i)$ via constructing a candidate set $\mathbb{U}$ from $\cup_{w \in \keyU(u_i)}\knnalg(w) \cup \pknnalg(u_i) \setminus \knnalg(u_i)$ in line 6. When there exists vertices in $\mathbb{U}$, we insert the vertex $v$ with smallest shortest distance into the end to $\knnalg(u_i)$ in lines 7-9.

\begin{algorithm}[htb]
        \caption{Query after Object Deletion}
        \label{alg:delete_tar}
        \DontPrintSemicolon            
            \KwInput{\knnindex after deleting $u$ and a query vertex $v$}
            \KwOutput{$\knnalg(v)$}
            $UG(v) \gets$ the upper graph of $v$;\;
            	\For{$i = l,..., 1$ in the reverse rank of $UG(v)$}{
            		\If{$u \notin \knnalg(u_i)$}{continue;}
            		delete $u$ from $\knnalg(u_i)$; \;
            		$\mathbb{U} \gets \cup_{w \in \keyU(u_i)} \knnalg(w) \cup \pknnalg(u_i) \setminus \knnalg(u_i)$; \;
            		\If{$\mathbb{U} \neq \emptyset$}{
            			$m \gets argmin_{m \in \mathbb{U}} \sd(m, u_i)$; \;
            			insert $m$ into the end of $\knnalg(u_i)$; \;
            		}
            }
            return $\knnalg(v)$;\;
\end{algorithm} 

\begin{theorem}
	Given the partial updated index of a graph $G$ and a deleted candidate vertex $u$, the time complexity of \refalg{delete_tar} is bounded by $O(l \cdot k \cdot f)$.
\end{theorem}

\proofsketch
	The size of $v$'s upper graph is bounded by $l$. In line 6, the size of $\mathbb{U}$ is $(|\keyU(u_i)| + 1) \cdot k \leq f \cdot k$. Therefore, the total time complexity of \refalg{delete_tar} is $O(l \cdot f \cdot k)$.
\eop

When there are many queries after deletes, the first part in the time complexity $O(l)$ is small in practice, since the upper graphs for these queries may exist intersections, in which the vertices do not need to be updated again. Especially, when the query vertex $u$ belongs to someone query vertex's upper graph,  $\knnalg(u)$ can directly be returned as the final answer.


\subsubsection{Simple Query after Deleting.}
Actually, not all query results after deleting some candidate objects would make changes. After deleting one object $v_{de}$ from $\mathcal{M}$, there are two situations for a query $\knnalg(v_q)$, respectively, $v_{de} \notin \knnalg(v_q)$ and $v_{de} \in \knnalg(v_q)$. For the first situation $v_{de} \notin \knnalg(v_q)$, the original $\knnalg(v_q)$ is the final answer. For the second situation $v_{de} \in \knnalg(v_q)$, there are two main cases. We use $v_k$ to represent the $k$th object in the original $\knnalg(v_q)$, and use $w_{k}$ to refer to the $k$th object in the original $\knnalg(w)$ ($w \in \keyU(v_q)$). When $v_k \notin U_k$, $U_k = \cup_{w \in \keyU(v_q)}\{ w_k \}$ and $dist(v_q,w_k) \neq dist(v_q,w) + dist(w,w_k)$, we directly scan all $\knnalg(w)$ ($w \in \keyU(v_q)$) and skip $v_d$ to calculate updated $\knnalg(v_q)$. Otherwise, when $v_k \in U_k$, $U_k = \cup_{w \in \keyU(v_q)}\{ w_k \}$ and $dist(v_q, w_k) = dist(v_q,w) + dist(w,w_k)$, we need to update $\knnalg(w)$ first. In this situation, the worst case is to start from scratch. However, in practice, the worst case happens occasionally.


\subsubsection{Candidate vertex Insertion.} The algorithm for inserting a candidate vertex is called \emph{KNN-Insert}, shown in \refalg{insert}.

In line 1, we collect $UG(u)$ for the inserted object $u$ and initialize the array $\psd(\cdot)$, which records the shortest peak distance between $u$ and each vertex in $UG(u)$. Notice that when a vertex $u$ is inserted into the candidate set, we only need to check whether the shortest peak distance between $u$ and $u_i$ is shorter than the distance between $v_k$ and $u_i$. Here, the vertex $v_k$ is the last vertex in $\pknnalg(u_i)$. In lines 3-4, we compute the shortest peak distance between $u$ and $w$. When $\psd[u_i] < \psd(u_i,v_k)$, we replace $w$ with $v_k$ in $\pknnalg(u_i)$ in lines 6-7. $\psd[u_i]$ is the shortest peak distance between $u_i$ and $u$. 

\begin{algorithm}[htb]
        \caption{\knn Insert}
        \label{alg:insert}
        \DontPrintSemicolon            
            \KwInput{\knnindex and a inserted vertex $u$}
            \KwOutput{The updated \knnindex}
            	$UG(u) \gets$ the upper graph of $u$;  $\psd(\cdot) \gets +\infty$;\;
            	\For{$i = 1,2,...,n$ in the ascending order of rank in $UG(u)$}{
            		\For{$w \in \keyU(u_i)$}{
            			$\psd[w] \gets min\{ \psd(u_i) + \sd(u_i,w), \psd[w] \}$;
            		}
                $v_k \gets$ the last vertex in $\pknnalg(u_i)$;\;
                \If{$\psd(u_i,v_k) > \psd[u_i]$}{
            replace $v_k$ with $u$ in $\pknnalg(u_i)$; \;
               }
            	}
\end{algorithm} 

\begin{theorem}
	Given \knn of a graph $G$ and an inserted candidate vertex $u$, the time complexity of \refalg{insert} is bounded by $O(l \cdot f)$.
\end{theorem}

\proofsketch
	According to \reflem{ugsize}, the size of upper graph for $u$ is bounded by $l$. In lines 3-4, the $\psd(\cdot)$ computation cost $O(f)$ time. The last vertex in $\pknnalg(u_i)$ can be grabbed in the constant time, since we store $\pknnalg(u_i)$ in the bidirectional linked array. Therefore, the total time complexity of \refalg{insert} is $O(l \cdot f)$.
\eop

%\subsubsection{Targeted-Index Update for Specific Queries.}

\subsubsection{Special Query after inserting objects} The algorithm for KNN query for $v$ after inserting a candidate vertex $u$ is shown in \refalg{insert_tar}.

In line 1, we construct $UG(v)$ for the query vertex $v$ and initialize the array $\sd(\cdot)$, which records the shortest distance between $u$ and each vertex in $UG(v)$. Notice that when a vertex $u$ is inserted into the candidate set, we only need to check whether the shortest distance between $u$ and $u_i$ is shorter than the distance between $v_k$ and $u_i$. Here, the vertex $v_k$ is the last vertex in $\knnalg(u_i)$. We compute the shortest distance between $u$ and $u_i$ in lines 3-4. When $\sd[u_i] < \sd(u_i,v_k)$, we replace $w$ with $v_k$ in $\knnalg(u_i)$ in lines 6-7. $\sd[u_i]$ is the shortest distance between $u_i$ and $u$. 

\begin{algorithm}[htb]
        \caption{Query after Object Insertion}
        \label{alg:insert_tar}
        \DontPrintSemicolon            
            \KwInput{\knn after inserting $u$ and a query vertex $v$}
            \KwOutput{$\knnalg(v)$}
            $UG(v) \gets$ the upper graph of $v$; $\sd(\cdot) \gets + \infty$; \;
            	\For{$i = l,... ,1$ in the descending order of rank in $UG(v)$}{
            		$\overline{\sd}(u_i,u) \gets \min_{w \in \keyU(u_i)} \{ \sd(u_i,w) + \sd[w] \}$; \;
            		$\sd[u_i] \gets min\{ \overline{\sd}(u_i,u), \psd[u_i]  \}$; \;
            		$v_k \gets$ the last vertex in $\knnalg(u_i)$;\;
            		\If{$dist(u_i,v_k) > dist[u_i]$}{
            			replace $v_k$ with $u$ in $\knnalg(u_i)$; \;
            		}
            	}
            return $\knnalg(v)$;\;
\end{algorithm} 

\begin{theorem}
	Given \knnindex of a graph $G$ and an inserted candidate object $u$, the time complexity of \refalg{insert_tar} is bounded by $O(l \cdot f)$.
\end{theorem}

\proofsketch
	Following \reflem{ugsize}, the size of upper graph for $u$ is bounded by $l$. In lines 3-4, the $\sd(\cdot)$ computation cost $O(f)$ time. The last vertex in $\knnalg(u_i)$ can be grabbed in the constant time, since we store $\knnalg(u_i)$ in the bidirectional linked array. Therefore, the total time complexity of \refalg{insert} is $O(l \cdot f)$.
\eop

\subsubsection{Simple Query after Inserting.}

When answering a query after inserting an object into the candidate set $\mathcal{M}$, it is unnecessary to update \knn for vertices with higher rank than $v_q$, since many them are not queried. In \refsec{exp}, we will show the frequency that vertices can reuse updated \knn, which is very low. So we can skip the step of updating \knn for vertices with higher ranks than $v_q$, which means we only update $\knnalg(v_q)$. To update exact and accurate \knn, we need to calculate the global shortest distance between $v_q$ and $v_{in}$ and then to compare $dist(v_q,v_{in})$ with $dist(v_q,v_k)$ from original $\knnalg(v_q)$. $v_k$ represents $k$th vertex in $\knnalg(v_q)$. Only when $dist(v_q,v_{in}) < dist(v_q,v_k)$, we need to insert $v_{in}$ to an accurate position of $\knnalg(v_q)$ and then delete the final one vertex. Otherwise, $\knnalg(v_q)$ is the direct answer.a 

==> con.tex <==
\section{Index Construction $\&$ Update}
\label{sec:indexcon}

Based on the structure of \knnindex, it can be constructed straightforwardly by computing the top $k$ nearest neighbors of each vertex through  \kw{Dijkstra's} algorithm or \tenindex. However, these approaches are time-consuming  (with time complexity  $O(n \cdot (m + n \cdot \log n ))$ or $O(n \cdot \log n + n \cdot h \cdot w + n \cdot h \cdot k)$ ). Obviously, these approaches are unscalable to handle large road network. In this section, we present our new approach to construct the \knnindex.

\subsection{Vertex Cut and $k$ Nearest Neighbor Distance}

The above discussed approaches compute the $k$ nearest neighbors for each vertex independently, which miss the potential opportunities to re-use the intermediate results during the construction. In this section, we introduce  an important observation regarding the vertex cut and shortest distance computation, which lay the foundation  of our computation-sharing index construction algorithm.

\label{sec:properties}
\begin{definition}
    \textbf{($u$ Vertex Cut)}
	\label{def:vc}
	Given a graph $G$, for a vertex $u$, a subset of vertices $VC(u) \subset V(G)$ is a vertex cut for $u$ if $u$ disconnects with any vertices of the graph $V(G)\setminus\{VC(u) \cup u\}$ after removing $VC(u)$ from $G$. 
\end{definition}
 

Based on \refdef{vc}, given a vertex $ u \in G$, for any vertex $v \in G$, the shortest path between $u$ and $v$ must pass at least one vertex $w \in VC(u)$.  Moreover, for $v \in R_k(u)$ and $v \notin VC(u)$, there exists at least one vertex $w \in VC(u)$ such that $v \in R_k(w)$. This is because if $v \in R_k(u)$  but $v \notin \cup_{w \in VC(u)} R_k(w)$. Then, there exists one $w \in VC(u)$ such that for all $v_i \in R_k(w)$, $1 \leq i  \leq k$, we have $dist(w,v_i) < dist(w,v)$.  Then $dist(u, w) + dist(w,v_i) < dist(u,w) + dist(w,v)$. It means there are at least $k$ vertices whose distance to $u$ is smaller than the distance between $u$ and $v$, which contradicts $v \in R_k(u)$. Based on this observation, we have the following property regarding the vertex cut and $k$ nearest neighbors: 


%Simply, the top-$k$ nearest neighbors search for a query vertex $u$ is to compute shortest distance between $u$ and other vertices in the graph and then to sort them in an ascending order of their shortest distance to $u$, finally to get the top $k$ vertices from them. So the essence of the classic KNN problem is how to achieve top $k$ vertices with the smallest shortest distance for every vertex in the road networks efficiently. Obviously, shortest distance computation is an essential part for dealing with the KNN problem. 

%From observation on the vertex cut definition, we get the following shortest distance reuse property, which can efficiently guarantee that our \knnindex is both correct and exact.


\begin{property}% ($v \notin CV(u)$)
\label{pro:computationsharing}
     Given a vertex $v \in R_k(u)$, we have $dist(u,v) = min_{w \in VC(u) \wedge v \in R_k(w)} \{ dist(v,w) + dist(w,u) \}$.  
\end{property}


Based on the structure of \knnindex, the key to construct the index is to obtain the shortest distance between a vertex $u$ and other vertices. As analyzed in the above, for a vertex $v$, if $v \in R_k(u)$, $v$ must be in $\cup_{w \in VC(u)}R_k(w)$. In other words, if we have known $R_k(w)$ for each vertex  $w \in VC(u)$, we can know the possible vertex set of $R_k(u)$. Following the similar idea, if we have known  $dist(w, u)$ and $dist(w, u)$ for $w \in VC(u), v \in R_k(w)$, we can obtain $dist(u, v)$ based on  \refpro{computationsharing} as well. Therefore, instead of computing the $k$ nearest neighbors together with their distance for each vertex individually, we can share the computed results to improve the construction performance. 

 %anyone vertex $u$, if all \knn(w) ($\forall w \in VC(u)$) computation are completed, then the distance information for \knn(u) can be achieved directly from the distance of \knn(w). We can get $dist(w,u)$ from the preprocessed graph directly. According to \refdef{vc}, the shortest path between any vertex $v$($v \notin VC(u)$) in $\knn(u)$ and $u$ must pass through at least one vertex $w$ ($w \in VC(u)$). For $dist(v,w)$, we can directly get it from \knn(w). Following this idea, we .



%So \refproperty{dsp} can expedite our index construction efficiently. In this way, 

%We next discuss about the effect of candidate set $\Omega$ for each vertex $u$ on computing \knnindex. It is easy to guarantee that each \knnindex only contains the vertices belonging to $\Omega$ under our index framework. Following \refproperty{vcp}, for each vertex $u$, if all $\knn(v) \subseteq \Omega$ ($v \in VC(u)$), \knn(u) must belong to $\Omega$.
%
%Based on above properties, we can get the total top-k nearest neighbors for each vertex on the graph efficiently.
%
%\stitle{\underline{Vertex Cut based Framework.}} Following above two properties, a straightforward method is to give a rank for all vertices. According to this rank, \kw{Dijkstra} search is used to calculate the top k nearest neighbors for each vertex $v \in VC(u)$ firstly. Then, \knnindex for $u$ can directly select from \knnindex of $VC(u)$ instead of conducting \kw{Dijkstra} from the scratch.

\subsection{A Vertex Cut based Construction Framework}
\label{sec:naive}

As discussed above, to achieve the goal of efficient index construction by sharing the computed results, the first problem we have to address is to compute a $u$ vertex cut $VC(u)$ for each vertex $u$. Moreover, we prefer to a smaller $VC(u)$ following \refpro{computationsharing} intuitively. Therefore, we first give a rank for each vertex as follows:

\begin{definition}
\label{def:vr}
\textbf{(Vertex Rank)} Given a road network $G$, for two vertex $u$ and $v$ in $G$, $u$ has a higher rank than $v$ if $\mydeg(u) > \mydeg(v)$. When $\mydeg(u) = \mydeg(v)$, $u$ has a higher rank than $v$ when $\myid(u)>\myid(v)$.
\end{definition}


For a vertex $u$, we use $rank(u)$ to denote its rank. Following \refdef{vr}, we use \refalg{vertexcutgen} to compute a vertex cut for each vertex. Specifically, we initializes $G'$ as the input road network $G$ (line 1). Then, we iterates the vertices in $G'$ in the increasing order of their ranks (line 3-9). For each $w_i$,  $VC(w_i)$ is set as the neighbors of $w_i$ in $G'$(line 3). Then, we further iterate the vertex pair $u, v$ in the  neighbors of $w_i$ such that $u$ and $v$ have a higher rank than $w_i$ (line 4). If the edge $(u, v)$ is not in $E(G')$, then we insert it in it and set the weight as $ \phi((u,w_i), G') + \phi((w_i,v), G')$ (line 6-7). Otherwise, if $\phi((u,w_i), G') + \phi((w_i,v), G') < \phi((u,v), G')$, then the weight of $(u, v)$ is updated to $\phi((u,w_i), G') + \phi((w_i,v), G')$ (line 9). The algorithm finishes when all the vertices have been explored (line 2). Note that in \refalg{vertexcutgen}, apart from the vertex cut, we also generates a weighted graph $G'$, which will be used to share the $k$ nearest neighbor distance computation afterwards. 

%in each iteration, we select the vertex according to the rank (line 2), $nbr^+(w)$ and $w$ form the future vertex cut $HV(w_i)$ (line 3).$nbr^-(w)$ form the past vertex cut $LV(w_i)$ (line 4). Lines 5-10 provides the foundation for next vertex and computes the partial shortest distance. For each vertex pair $(u,v)$ for vertices in $nbr^+(w_i)$, if $e(u,v)$ does not exist in $G$, $e(u,v)$ will be added into $G$ and the weight (partial shortest distance) of $e(u,v)$ is also calculated (lines 6-8). Otherwise, when $e(u,v)$ already exists in $G$, if the weight of $e(u,v)$, $\phi(u,v)$, is not equal to their partial shortest distance, the weight of $e(u,v)$ will be updated as $\phi(u,w_i) + \phi(w_i,v)$.

\begin{algorithm}[htb]
        \caption{Vertex-Cut Graph Generation}
        \label{alg:vertexcutgen}
        \DontPrintSemicolon
        \KwInput{A road network $G$}
        \KwOutput{Vertex cut for each vertex}
        %Give a rank for all vertices in $G$; \;
        $G' \gets G$;\;
        \ForEach{$w_i \in V(G')$ in the increasing order of their ranks }{
            $VC(w_i) \gets \nbr(w_i, G')$;\;            
            \For{all pairs of vertices $u,v \in nbr(w_i, G')$ with higher rank than $w_i$}{
            		\If{$(u,v) \notin E(G')$}{
               		insert $(u,v)$ into $G'$;\;
               		$\phi((u,v), G') \gets \phi((u,w_i), G') + \phi((w_i,v), G')$; \;
            		}\ElseIf{$\phi((u,w_i), G') + \phi((w_i,v), G') < \phi((u,v), G')$}{
                		$\phi((u,v), G') \gets \phi((u,w_i), G') + \phi((w_i,v), G')$; \;
            		}
        	}
        }
\end{algorithm} 


It is obvious $VC(\cdot)$ assigned to each vertex in line 3 of the \refalg{vertexcutgen} is a $u$ vertex cut following \refdef{vc}. To facilitate the index construction, we further divide $VC(u)$ into two sets: lower vertex cut $LV(u)$  which contains the vertices in $VC(u)$ with lower ranks than $u$, and higher vertex cut $HV(u)$ which contains the vertices in $VC(u)$ with higher ranks than $u$. The following problem is how to efficiently compute the shortest distances to obtain the $k$ nearest neighbors. Before introducing our algorithm, we first define:  

%\begin{lemma}
%    \label{lem:vcfp}	
%%    Given each vertex $u$ in $G'$, $LV(u) \cup HV(u) = VC(u)$.
%\end{lemma}
%
%\proofsketch
%   Definitely, after deleting $LV(u)$, $u$ cannot connect to the vertices with lower rank than $u$ in $G_{SPD}$. And after deleting $HV(u)$, $u$ cannot connect to the vertices with higher rank than $u$ in $G_{SPD}$. When deleting $LV(u)$ and $HV(u)$, $u$ disconnects with any vertices of the graph $G_{SPD}$. So, $PV(u) \cup FV(u) = VC(u)$.
%\eop


%a straightforward method is to give a rank for all vertices. According to this rank, \kw{Dijkstra} search is used to calculate the top k nearest neighbors for each vertex $v \in VC(u)$ firstly. Then, \knnindex for $u$ can directly select from \knnindex of $VC(u)$ instead of conducting \kw{Dijkstra} from the scratch.
 
%Even if above vertex cut based framework works, \kw{Dijkstra} for a part of vertices still causes long indexing time. These \kw{Dijkstra} search exists too much repetition, which means some distance are repeatedly calculated. 


%To make full use of vertex cut property and distance reuse property, we seperate $VC(\cdot)$ into two disjoint set, $LV(\cdot)$ and $HV(\cdot)$ according to the given rank and adapt two steps to complete the index construction efficiently and effectively. 
%
%Specifically, $LV(u)$ denoted the rank lower neighbors of $u$, $HV(u)$ denoted the rank higher neighbors of $u$. The first \knnindex construction step is to adapt a Low-to-High manner, which uses $LV(u)$ to collect the partial \knnindex from the sub-candidate objects, whose rank is lower than $u$, we record the partial KNN as \pknn($u$) index. And the second step is to utilize a High-to-Low manner, which makes use of $HV(u)$ to collect objects with higher ranks and aggregates $\pknn(u)$ to achieve the final total \knnindex. 

%To achieve exact and correct \knnindex via $LV(u)$ and $HV(u)$, $LV(u)$ and $HV(u)$ generation becomes the foundation for our \knnindex construction. Next, we will introduce how to generate $LV(u)$ and $HV(u)$ in \refsec{vc}. And we will show the first \knnindex construction step in \refsec{first} and the second step in \refsec{second}.

%\subsubsection{Step0: Vertex Cut Generation}
%\label{sec:vc}

%A straightforward method is to directly achieve vertex cut from the original graph for each vertex. Just for a given graph, and then we give a rank for all vertices. For each vertex $u$, divide $nbr(u)$ into two disjoint vertex sets, respectively $nbr^+(u) (LV(u))$ and $nbr^-(u) (HV(u))$. But if we do so, we will miss important shortest distance between $u$ and anyone vertex $v$, which passes through one vertex in $LV(u)$. So we cannot generate $LV(\cdot)$ and $HV(\cdot)$ in this easy but wrong way.
%
%To avoid missing necessary distance, every time we generate $LV(u)$ and $HV(u)$ for a vertex $u$, we need to add an edge for each pair of $nbr^+(u)$ if there is not an edge; otherwise, we need to check whether the weight of this edge needs to be updated.  
%
%When generating vertex cut, we also record the weight for each new added edge and each one with an updated weight, especially shown in lines 5-10 of \refalg{treedecom}, which does not affect the time consumption at all. We will explain this in the time complexity analysis in \refthm{cutgen}.

\begin{definition}
	\textbf{Partial Path.} Given a road network $G$, for any two vertices $v$ and $u$, there exists many partial path such that $v, v_1, v_2,..., v_n, u$, $rank(v_i) < min(rank(v), rank(u)), i \in [1,n]$, denoted as $pp(v,u)$.
\end{definition}

\begin{definition}
	\textbf{Partial Shortest Distance.} Given a road network $G$, for any two vertices $v$ and $u$, the partial shortest distance is the shortest distance from all $pp(v,u)$, denoted as $psd(v,u)$.
\end{definition}

%After generating vertex cut, we can achieve the PSDP-Graph $G_{PSD}$ for the input road network $G$ as an additional result.

Recall the graph $G'$ generated in \refalg{vertexcutgen}. Obviously, we have the following lemma:

\begin{lemma}
\label{lem:psdp}
Given the graph $G'$ generated in \refalg{vertexcutgen}, for each $e = (u, v) \in E(G')$, we have $\phi((u, v), G') = psd(u, v)$.	
\end{lemma}

According to \reflem{psdp}, $G'$ preserves the partial shortest distance in the input road network $G$. For the clearness of presentation, we call $G'$ {P}artial \underline{S}hortest \underline{D}istance \underline{P}reserved Graph (PSDP-Graph), and denote it as $G_{PSD}$.


%\begin{definition}
%	\textbf{PSDP-Graph.} Given a road network $G$, a graph $G_{PSD}$ is a \underline{P}artial \underline{S}hortest \underline{D}istance \underline{P}reserved Graph (PSDP-Graph) such that $\forall e = (u,v) \in E(G_{PSD})$, $\phi(u,v) = psd(u,v)$.
%\end{definition}



\begin{figure}
    \centering
    \includegraphics[width=0.70\linewidth]{fig/PSD_Graph.pdf}
    \vspace{-0.2cm}
    \caption{$G_{PSD}$ of $G$}
    %\vspace{-0.4cm}
    \label{fig:PSD_G}
\end{figure}


\begin{example}
    \reffig{PSD_G} shows the partial shortest distance preserved graph. Take $v_8$ as an example, $VC(v_8) = \left\{ v_2, v_6, v_7, v_9, v_{20} \right\}$, we can achieve $LV(v_8) = \left\{ v_2, v_6, v_7 \right\}$ and $HV(v_8) = \left\{ v_9, v_{20} \right\}$.
\end{example}

%\stitle{Algorithm.} \refalg{treedecom} shows the procedure of generating vertex cut. Firstly, we compute a rank for each vertex in graph(line 1). In each iteration, we select the vertex according to the rank (line 2), $nbr^+(w)$ and $w$ form the future vertex cut $HV(w_i)$ (line 3).$nbr^-(w)$ form the past vertex cut $LV(w_i)$ (line 4). Lines 5-10 provides the foundation for next vertex and computes the partial shortest distance. For each vertex pair $(u,v)$ for vertices in $nbr^+(w_i)$, if $e(u,v)$ does not exist in $G$, $e(u,v)$ will be added into $G$ and the weight (partial shortest distance) of $e(u,v)$ is also calculated (lines 6-8). Otherwise, when $e(u,v)$ already exists in $G$, if the weight of $e(u,v)$, $\phi(u,v)$, is not equal to their partial shortest distance, the weight of $e(u,v)$ will be updated as $\phi(u,w_i) + \phi(w_i,v)$.
 
 
With the PSDP-Graph, we can construct \knnindex  in two steps:

\subsubsection{Step1: \pknnindex construction with Upper Bound Distance}
\label{sec:first}

To make full use of distance reuse property, the aim of \pknn Index is to use $LV(u)$ to collect all possible candidate objects with lower rank than $u$. When the size of these candidate objects is larger than $k$, we use the partial shortest distance to filer top k objects with partial shortest distance.


\begin{definition}
	\textbf{\underline{P}artial top-\underline{K} \underline{N}earest \underline{N}eighbors Index (\pknnindex).} we call the top-k vertices in ascending order of partial shortest distance to $u$ as its \pknnindex, denoted as $\pknnalg(u)$. $\pknnalg(u)\subseteqq (\mathcal{M} \cap \{u\}) \bigcup_{w \in LV(u)} \pknnalg(w)$.
\end{definition}


\begin{lemma}
    \label{lem:pathFirstAndSec}
	For any two vertices $u,v \in G$, arbitrary one shortest path $SPath(u,v) = {u,w_0,w_1,...w_k,v}$, the vertex $w_i$ has the highest rank in $SPath$ and let $w_j$ has the second highest rank in $SPath$. We have $w_i \in HV(w_j)$.
\end{lemma}

\proofsketch
Recall that we introduce our vertex cut generation algorithm in \refalg{vertexcutgen}. Let $w$ be the vertex with the lowest rank in $SPath(u,v)$. Let $w_l$ and $w_r$ be the previous and the next vertex of $w$ in the path. During the procedure of vertex cut generation, after generating vertex cut for $w$, we will connect $w_l$ and $w_r$. As a result, $w_l$ and $w_r$ are connected. It follows that $w_i \in HV(w_j)$ after processing $w_j$.
\eop

\begin{lemma}
    \label{lem:oneDist}
	For each vertex $u$, from $HV(u)$, at least one vertex $v$($v \in HV(u)$) has the shortest distance with $u$, namely, $ \phi((u,v),G') = dist(u,v)$. 
\end{lemma}

%the rank of $p$ is lower than the rank of $u$
\proofsketch
Anyone shortest path between any two vertices $u$ and $v$ in $G$ must pass at least one vertex $w$, $w \in nbr(u)$. We assume that there is not a vertex $v$ ($v \in HV(u)$ or ($v \in nbr^+(u)$)) such that $\phi((u,v),G') = dist(u,v)$. $SPath(u,v)$ must pass through one vertex $v^- \in nbr^-(u)$. So if $PP(u,v) = SPath(u,v)$, $\phi((u,v),G') = dist(u,v)$, which contradicts the assumption. Otherwise, $SPath(u,v)$ must pass a vertex $v$,($v \in nbr^+(u)$), which contradicts the assumption, so the proof completes.
\eop

%\proofsketch
%	We proof it by induction. For the base case, 
    %We proof it by induction. For the base case depth(u) = 1, the lemma holds obviously. Assume the lemma holds for depth(u) = i, and then depth(u) = i+1,
    %When anyone vertex $u$, ($depth(u) \in [0,h]$), 
    %For any pair of vertices $u$ and $v$ (assuming that depth(u) $>$ depth(v) and $v \in X(u)$), a shortest path between them in the road network is $u, w_1, w_2,..., w_n, v$, $w_1$ must exist in $X(u)$ and dist(u,$w_1$) is global shortest distance.
    %If the distance of $u$ and $v$ ($v \in X(u)$) is partial shortest distance, there is at least one vertex $w$ ($w \in X(u) \setminus {v}$) such that $dist(u,v) = dist(u,w) + dist(w,v)$ (1). Assume that $dist(u,v)$ and $dist(u,w)$ are both partial distance, which means $dist(u,w) = dist(u,v) + dist(w,v)$ (2). If (1) and (2) exist at the same time, we can get $dist(w,v) =0$, which does not appear in the graph. $dist(w,v) =0$ contradicts the assumption.
%\eop

\begin{lemma}
	For each vertex $u$ in $G$, if $v \in \pknnalg(u)$, there must be a vertex $w \in LV(u)$ such that $v \in \pknnalg(w)$.
\end{lemma}

\proofsketch
    Assume the opposite, there exists a vertex $v \in \pknnalg(u)$, but $v \notin \pknnalg(w)$, $w \in LV(u)$. Based on \refdef{vc}, we can get at least one vertex $w$ ($w \in LV(u)$), such that $dist(u,v) = dist(u,w) + dist(w,v)$. The distance between $k$th vertex in \pknn(w) and $w$ is $dist_{pk}(w)$, such that $dist_{pk}(w) < dist(w,v)$. Then $dist(u,v) = dist(u,w) + dist(w,v) > dist_{pk}(w) + dist(u,w)$, which means that there are at least k vertices with smaller partial shortest distance than $v$ to $u$. This contradicts the assumption.
\eop

The difference between \pknnindex and \knnindex is from two aspects: 1. whether the distance between $u$ and $v \in KNN(u)$ is the global shortest distance in $G$; 2. whether the possible candidate set can cover all objects in $\mathcal{M}$. For the final $\knnalg(u)$, the shortest paths between $u$ and top k nearest neighbors must pass through at least one vertex in either $LV(u)$ or in $HV(u)$. Also, we grab objects with lower rank than $u$ via $LV(u)$ and get objects ranker higher than $u$ via $HV(u)$. To cover all objects in $\mathcal{M}$ and to achieve the shortest distance, all vertices in $LV(u)$ and $HV(u)$ should be explored. So we can conclude that when all vertices in the vertex cut are explored, the exact and correct top k nearest neighbors with shortest distance can be achieved.

\begin{lemma}
	For the rank highest vertex $v_n$, $\pknnalg(u_n)$ is equal to $\knnalg(u_n)$.
\end{lemma}

\proofsketch
    For the vertex $v_n$, $LV(u_n)$ is not only the lower vertex cut but also the whole vertex cut for $v_n$, namely $LV(u_n) = VC(u_n)$.  
\eop


\begin{example}
    We can compute $\pknnalg(v_{20}) = \{v_{20}, v_9, v_8, v_7, v_{14} \}$, which is the same as $\knnalg(v_{20})$, shown in \reffig{VCGKNN}.
\end{example}


\subsubsection{Step2: \knnindex Construction with Shortest Distance}
\label{sec:second}

\begin{lemma}
    For each vertex $u$, if $v \in \knnalg(u)$, there is a vertex $w \in HV(u)$ such that $v \in \knnalg(w)$ or $v \in \pknnalg(u)$, namely, $\knnalg(u) \subseteq (\pknnalg(u) \bigcup$ $(\bigcup_{w \in 
    HV(u)} \knnalg(w)))$.   
\end{lemma}

\proofsketch
According to \refproperty{computationsharing}, $\forall v \in R_k(u)$, $SPath(v,u)$ must pass through one vertex $w$ ($w \in VC(u)$). $\pknnalg(u)$ contains all $v$, whose $SPath(v,u)$ pass through $LV(u)$. $\bigcup_{w \in 
    HV(u)} \knnalg(w)$ contains all $v$, whose $SPath(v,u)$ pass through one vertex $w$ ($w \in HV(u)$). So $\knnalg(u) \subseteq (\pknnalg(u) \bigcup$ $(\bigcup_{w \in 
    HV(u)} \knnalg(w)))$.
\eop
%\proofsketch
    %We proof this lemma via its contradiction. Assuming that $v \in VCT(u)$ (Assumption A), $v \notin VCP(u)$ (Condition B) and $v \notin VCT(p) (p \in FV(u))$ (Condition C). With A and B, which means that a shortest path between u and v must pass through a vertex $p$ in the future vertex cut $FV(u)$, such that $dist(u,v) = dist(u,p) + dist(p,v)$ and $dist(u,v) < dist_k(u)$ . With condition C, we can get that $dist(p,v) > dist_k(p)$. Then, $dist(u,p) + dist(p,v) > dist(u,p) + dist_k(p)$ shows that there are at least k vertices to $u$ with the smaller distance than $v$, which contradicts the assumption A. The proof finishes.
%\eop



\begin{algorithm}[htb]
    \caption{A \knnindex construction}
    \label{alg:naiveindexcon}
    \DontPrintSemicolon
        \KwInput{A Road Network G}
        \KwOutput{KNN index}
        Generate vertex cut and record $G_{PSDP}$ of $G$ ; \;
        $C \gets \emptyset$, $\pknnalg(\cdot) \gets \emptyset$, $\knnalg(\cdot) \gets \emptyset$; \; 
        \ForEach{$i = 1,2,...,n$}{
            $C \gets \mathcal{M} \cap \{ u_i \}$; \;
            \ForEach{$w \in LV(u_i)$}{
                $C \gets C \cup \pknnalg(w)$;
                $\overline{dist}(u_i,w) \gets \phi(u_i,w)$;
            }
            \ForEach{$v \in C$}{
            $ \overline{dist}(u_i,v) \gets \min_{w \in LV(u_i)} \overline{dist}(u_i,w) + \overline{dist}(w,v); $ \;
            }
            sort vertices in $C$; \;
            $\pknnalg(u)$ $\gets$ top-k nearest vertices in $C$; \;
        }
        \ForEach{$i = n, n-1,...,1$}{
            $C \gets$ $\pknnalg(u_i)$; \;
            \ForEach{$w \in HV(u_i)$}{
                $C \gets C \cup \knnalg(w)$;
                $\overline{dist}(u_i,w) \gets \phi(u_i,w)$;
            }
            \ForEach{$v \in C$}{
            $ dist(u_i,v) \gets \min_{w \in HV(u_i)} \overline{dist}(u_i,w) + \overline{dist}(w,v)$; \;
            }
            sort vertices in $C$; \;
            $\knnalg(u) \gets$ top-k nearest vertices in $C$; \; 
            }
        return $\knnalg(\cdot)$; \;
        
\end{algorithm}


\stitle{Algorithm.} \refalg{naiveindexcon} shows the process for $\knnalg(\cdot)$ construction. Line 1 is the procedure of generating vertex cut (\refalg{vertexcutgen}). Lines 3-10 follow \underline{\emph{the step 1}} to construct $\pknnalg(\cdot)$. Line 4 guarantees that $\pknnalg(u_i)$ only contains objects in $\mathcal{M}$. Lines 4-5 push all possible objects into set $C$, $C$ is a candidate set for $\pknnalg(\cdot)$. Based on \refproperty{computationsharing}, Lines 7-8 compute the partial shortest distance for each vertex in $C$. Line 9 sorts them via the partial shortest distance. Line 10 selects top k nearest vertices from $C$ as $\pknnalg(u_i)$. Lines 11-18 represents \underline{\emph{the step 2}} to construct $\knnalg(\cdot)$. Lines 12-14 put $\pknnalg(u_i)$ and $\knnalg(w)$ ($\forall w \in HV(u_i)$) into $C$. Lines 15-16 follow \refproperty{computationsharing} to calculate shortest distance between $u_i$ and $w$ ($w \in HV(u_i)$). Lines 17-18 sort them via shortest distance and then grab top-k vertices as the finial $\knnalg(u_i)$. 



\begin{figure}[htb]
 \vspace{-0.1cm}
  \centering
   \subfigcapskip=0pt
   \subfigcaptopadj=0pt
   \subfigure[\pknnindex$(v_8)$]
   	 { \includegraphics[width=0.45\linewidth]{fig/KNN_CON_UP.pdf}
       \label{fig:KNN_CON_UP}}
 \subfigure[\knnindex$(v_8)$]{ \includegraphics[width=0.45\linewidth]{fig/KNN_CON_DOWN.pdf}
 	   \label{fig:KNN_CON_DOWN}
	 }
  \vspace{-0.1cm}
 \caption{\knnindex Construction}
  \label{fig:naive_con}
\end{figure}


\begin{example}
\emph{Step0: vertex cut identification for $v_8$.}
In \reffig{PSD_G}, we take $v_8$ as an example. $LV(v_8) = \{ v_2, v_6, v_7 | 3,8,5 \}$ and $HV(v_8) = \{ v_9, v_{20} | 5,2 \}$. 


\emph{Step1: \pknnindex construction for $v_8$.}
As \reffig{KNN_CON_UP} shown, $\pknnalg(v_6)=\{ v_6, v_1, v_2|0,3,5 \}$, $\pknnalg(v_7)=\{ v_7, v_6, v_1, v_2|0,2,5,7 \}$ and $\pknnalg(v_2)=\{ v_2, v_1| 0, 2\}$. We can get $C = \{v_8, v_2, v_1, v_7, v_6 | 0,3,5,5,7\}$. Finally, $\pknnalg(v_8) = \{ v_8, v_2, v_1, v_7, v_6 \}$.

\emph{Step2: \knnindex construction for $v_8$.}

As \reffig{KNN_CON_DOWN} shown, $\knnalg(v_9) = \{ v{9},v_{20},v_{19},v_7,v_8 | 0,1,2,3,3,3 \}$, $\pknnalg(v_{20}) =\{ v_{20},v_9,v_7,v_8,v_{14},v_{19} | 0,1,2,2,3,3 \}$. We can achieve that $C = \{v_8, v_{20}, v_2, v_9, v_1, v_7, v_{11} ,v_{14} ,v_{19} | 0,2,3,3,4,4,5,5,5\}$. From $C$, we can get $\knnalg(v_8) = \{ v_8, v_{20}, v_2, v_9, v_1\}$.
\end{example}

\begin{theorem}
\label{thm:cutgen}
	The vertex cut generation needs $O( n \cdot f^2)$ ($f = max_{v \in V}|LV(v)|$).
\end{theorem}

\proofsketch
   Lines 3 in \refalg{vertexcutgen} needs $O(f)$, line 4, for each vertex, it will be scanned $O(f)$. Lines 2-4 the time complexity is bounded by $O(n \cdot f)$. Adding edges and updating weight costs $O(f^2)$(Lines 5-10). Overall, the time complexity is $O(n \cdot f^2)$.
\eop


\begin{theorem}
	The time complexity of \knnindex construction is bounded by $O(n \cdot f^2 + n \cdot f \cdot k)$ ($f = max_{v \in V}|HV(v)|$).
\end{theorem}

\proofsketch
    Refer to \refthm{cutgen}, we notice that the time complexity of vertex cut generation is $O(n \cdot f^2)$(line 1). For each vertex, they can be scanned $O(f)$ times, so the time complexity (lines 5,6) is $O(f \cdot k)$. The distance upper bound calculation (lines 7,8) and candidates selection (lines 5,6) can be done simultaneously. Overall, the time complexity (lines 3-10) is $O(n \cdot f \cdot k)$. Similarly, lines 11-18 can be bounded by $O(n \cdot f \cdot k)$. So $\knnindex$ construction can be bounded by $O(n \cdot f^2 + n \cdot f \cdot k)$.
\eop


\subsection{Vertex Cut Optimized Index Construction}
\label{sec:pro}
%Even though above method can avoid some redundant distance computation, there are 
%Our progressive method not only avoids duplicate distance computation(using upper bound distance or distance dependance property), but also omits distance computation for unnecessary vertices(get only one every time).
Using the vertex cut, \refalg{naiveindexcon} well shares the distance computation in the index construction and achieves significant speedup compared with computing the $k$ nearest neighbors by \kw{Dijkstra}'s algorithm or \tenindex individually.  In this section, we optimize the size vertex cut to further improve the index construction performance. We first define:
 

\begin{definition}
	\textbf{Key Low Vertex Cut.} When $v \in LV(u)$ and $\phi(u,v) = dist(u,v)$, we call them as \underline{k}ey \underline{L}ow \underline{v}ertex cut (KLV).
	\label{def:kpv}
\end{definition}

\begin{definition}
	\textbf{Key High Vertex Cut.} When $v \in HV(u)$ and $\phi(u,v) = dist(u,v)$, we call them as \underline{k}ey \underline{H}igh \underline{v}ertex cut (KHV).
	\label{def:kfv}
\end{definition}

\begin{lemma}
	For each vertex $u$ and $HV(u) \neq \emptyset$, minimum size of its key further cut is 1, namely, $\forall u \in V, |KHV(u)| \geq 1$.
\end{lemma}

\proofsketch

\eop


Following the above definitions \refdef{kpv} and \refdef{kfv}, we can achieve the following property.

\begin{property}
\label{property:}
	$\forall v \in \knnalg(u)$, each $w$ ($w \in KLV(u) \cup KHV(u)$) must be passed by at least one shortest path between $v$ and $u$.
\end{property}

\begin{lemma}
	For a vertex $u$, $v$ is the nearest object of $u$ in the $\knnalg(u)$, there must be at least one vertex $w$ ($w \in HV(u) \cup {u}$), such that $v$ is the nearest object in $\knnalg(w)$. When $w$ is $u$, $v$ is the nearest object in $\pknnalg(w)$. And $dist(u,v) = dist(u,w) + dist(w,v)$. 
\end{lemma}

\proofsketch
    Let the vertex $v$ be the nearest object of $u$ in the graph. According to \refproperty{computationsharing}, there exists at least one vertex $w$ ($w \in VC(u)$), $dist(u,v) = dist(u,w) + dist(w,v)$. We will proof it via following two folds:
    (1) When $w \in LV(u)$, $v$ is the nearest object of $u$ in $\pknnalg(u)$. Since $w \in LV(u)$, in $\pknnalg(u)$ $dist(u,v)$ is the shortest distance instead of the upper bound distance. 
    (2) When $w \in HV(u)$, $v$ is the nearest object of $w$ in the $\knnalg(w)$. We proof this in the opposite. Assume $v$ is not the  first one in the $\knnalg(w)$, the first one is $v_1$. So we have $dist(v,w) < dist(v_1,w)$, then $dist(v,w) + dist(w,u) < dist(v_1,w) + dist(w,u)$. Definitely, $v$ is not the nearest object of $u$, which contradict the condition.
    Overall, our proof finishes.
\eop
 
 
\begin{algorithm}[!tb]
        \caption{\knn$^*$-Index Construction}
        \label{alg:proindexcon}
        \DontPrintSemicolon           
            \KwInput{A Road Network G, A candidate set $\mathcal{M}$, an integer $k$}
            \KwOutput{\knnindex}
            Generate vertex cut and record $G_{PSDP}$ of $G$; \;
            $\knnalgpro(\cdot) \gets \emptyset; \pknnalgpro(\cdot) \gets \emptyset;$\;
            \ForEach{$ i = 1,2,...,n $}{
                $Q \gets \mathcal{M} \bigcap \{ u_i \}$;  $j \gets 1$;  \;
                %$rank_{max} \gets 0$;\;
                \ForEach{$w \in KLV(u_i)$}{
                    $pos[w] \gets 1$;
                    $dist[w] \gets \phi(u_i,w)$;\;
                    $pDist(w,pos[w],dist$); \;
                    %$rank_{max} \gets max(rank_{max}, rank(w))$;\;
                }
                \While{$j \leq k$ and $Q \neq \emptyset$}{
                    $v \gets$ Q.pop(); \;
                    $\pknnalgpro(u_i)$.push(v); \;
                    $pDist(vc[v],pos[vc[v]],dist)$; \;
                    $j \gets j+1$; \;
                }
            }
            \ForEach{$i = n,n-1,...,1$}{
                $dist[u_i] \gets 0$; $pos[u_i] \gets 1$;\;
                $j \gets 1$; $Q \gets \emptyset$; \;
                $pDist(u_i,pos[u_i],dist)$; \;
                \ForEach{$w \in KHV(u_i)$}{
                    $pos[w] \gets 1$;
                    $dist[w] \gets \phi(u_i,w)$;\;
                    $gDist(w,pos[w],dist)$; \;            
                }
                \While{$j \leq k$ and $Q \neq \emptyset$}{
                    v $\gets$ Q.pop(); \;
                    $\knnalgpro(u_i)$.push(n); \;
                    \If{$vc[v] = u_i$}{
                        $pDist(vc[v],pos[vc[v]],dist$); \;
                    }\Else{
                       $gDist(vc[v],pos[vc[v]],dist$); \;
                    }
                    $j \gets j+1$; \;
                }
            }
            return $\knnalgpro(\cdot)$; \;
\end{algorithm} 

\begin{algorithm}[htb]
    \caption{$pDist$ and $gDist$ Computation}
    \label{alg:distCom}
    \DontPrintSemicolon
            \myproc{$pDist$($w,pos[w],dist$)}{
                \While{$pos[w] \leq \pknnalgpro(w).length$}{
                    $m \gets \pknnalgpro(w)[pos[v]]$; \;
                    $curDist \gets dist[w] + \overline{dist}(w,m)$; \;
                    \If{$dist[m] = \infty$}{
                        $dist[m] \gets curDist$; \;
                        Break; \;
                    }\ElseIf{$dist[m] > curDist$}{
                        $dist[m] \gets curDist$;                     
                        $pos[w] \gets pos[w]+1$; \;
                    }\Else{
                        $pos[w] \gets pos[w]+1$; \;
                    }
                }
                \If{$pos[w] \leq \pknnalgpro(w).length$}{
                    Q.push(m);
                    vc[m] $\gets $ w;
                }
             }
             \myproc{$gDist$($w,pos[w],dist$)}{
                \While{$pos[w] \leq \knnalgpro(w).length$}{
                    $m \gets \knnalgpro(w)[pos[w]]$; \;
                    $curDist \gets dist[w] + \overline{dist}(w,m)$; \;
                    \If{$dist[m] = \infty$}{
                        $dist[m] \gets curDist$; \;
                        Break; \;
                    }\ElseIf{$dist[m] > curDist$}{
                        $dist[m] \gets curDist$;                     
                        $pos[w] \gets pos[w]+1$; \;
                    }\Else{
                        $pos[w] \gets pos[w]+1$; \;
                    }
                }
                \If{$pos[w] \leq \knnalgpro(w).length$}{
                    Q.push(m);
                    vc[m] $\gets $ v;
                }
             }	
\end{algorithm}
 
\stitle{Algorithm.} \refalg{proindexcon} shows the process for $\knnalgpro(\cdot)$ construction. Line 1 is \underline{\emph{the step 0}}, the procedure of generating vertex cut \refalg{vertexcutgen}. Lines 3-14 follow \underline{\emph{the step 1}} to construct $\pknnalgpro(\cdot)$. Line 4 guarantees that $\pknnalgpro(u_i)$ only contains objects in $\mathcal{M}$. Lines 5-7 collect first un-iterated vertex $m$ ($m \in \pknnalgpro(w), w \in KLV(u_i)$) and record the position where $m$ exists in $m \in \pknnalgpro(w)$. Lines 8-12 compute $\pknnalgpro(u_i)$. Lines 13-27 represent \underline{\emph{the step 2}} to construct $\knnalgpro(\cdot)$. Lines 14-19 select the first un-iterated vertex from $\pknnalgpro(u_i)$ and $\knnalgpro(w)$ ($\forall w \in KHV(u_i)$) into $Q$. Lines 20-26 compute $\knnalgpro(u_i)$.



\begin{figure}[htb]
 \vspace{-0.1cm}
  \centering
   \subfigcapskip=0pt
   \subfigcaptopadj=0pt
   \subfigure[\pknn$^*$-Index$(v_8)$]{ \includegraphics[width=0.45\linewidth]{fig/UP_PRO.pdf}
       \label{fig:UP_PRO}}
 \subfigure[\knn$^*$-Index$(v_8)$]{ \includegraphics[width=0.45\linewidth]{fig/DOWN_PRO.pdf}
 	   \label{fig:DOWN_PRO}
	 }
  \vspace{-0.1cm}
 \caption{\knn$^*$-Index Construction}
  \label{fig:naive_con}
  %\vspace{-0.1cm}
\end{figure}


\begin{example} 
\emph{Step0: key vertex cut identification for $v_8$.} In \reffig{PSD_G}, we take $v_8$ as an example. $KLV(v_8) = \{ v_2,v_7 | 3,5 \}$ and $KHV(v_8) = \{ v_{20} | 2 \}$.

\emph{Step1: \pknn$^*$-Index construction.}
As \reffig{UP_PRO} shown, $\pknnalgpro(v_2)=\{ v_2, v_1 | 0, 2\}$, $\pknnalgpro(v_7)=\{ v_7, v_6, v_1, v_2 | 0,2,5,7 \}$. After achieving the first vertex from $\pknnalgpro$ of $KLV(v_8)$, we get $Q = \{v_8, v_2, v_7 | 0,3,5 \}$. $dist[v_8]$ is minimized, so this first one popped from $Q$ is $v_8$. Then, Q pops $v_2$. Since $v_2$ from $\pknnalg(v_2)$, the next one $v_1$ from $\pknnalgpro(v_2)$ is pushed into $Q$, and $dist[v_1] = dist[v_2]+ \overline{dist}(v_2,v_1) = 5$. Now, $Q = \{v_1, v_7 | 5,5 \}$. Then, the third one popped from Q is $v_1$, since all vertices in $\pknnalgpro(v_2)$ are scanned, so no vertex is added into $Q$ now. The $4^{th}$ nearest objects is $v_7$. $v_7$ come from $\pknnalgpro(v_7)$, so $v_6$ is pushed into $Q$ with $dist[v_6] = dist[v_7] + dist(v_7,v_6) = 7$. Then, $Q = \{ v_6 | 7 \}$. Continue to pop $v_6$. $v_6$ is from $\pknnalgpro(v_7)$, next vertices are $v_2$ and $v_1$ in $\pknnalgpro(v_7)$. Since they are both scanned and has been put into $P_k(v_8)$, so they will not be added into $Q$ any more. So $Q$ is empty now, \pknn$^*$-Index construction for $v_8$ finishes. $\pknnalgpro(v_8) = \{ v_8, v_2, v_1, v_7, v_6 \}$.

\emph{Step2: \knn$^*$-Index construction.}
As \reffig{KNN_CON_DOWN} shows, $\pknnalgpro(v_8) = \{ v_8, v_2, v_1, v_7, v_6 | 0,3,5,5,7 \}$, $\knnalgpro(v_{20}) =\{ v_{20},v_9,v_7,v_8,v_{14} | 0,1,2,2,3\}$. We can get $Q = \{v_8, v_{20}| 0,2\}$. $v_8$ is popped, since it has smallest distance to $v_8$. $v_8$ is from $\pknnalgpro(v_8)$, $v_2$ with $dist[v_2] = dist[v_8] + \overline{dist}(v_8,v_2) = 3$ is pushed into $Q$. Now $Q =\{ v_{20},v_2| 2,3 \}$. The second vertex popped from $Q$ is $v_{20}$. $v_{20}$ is from $\knnalgpro(v_{20})$, $v_9$ is pushed into $Q$ with $dist[v_9] = dist[v_{20}] + \overline{dist}(v_{20},v_9) = 3$. Now $Q = \{ v_2, v_9| 3,3 \}$, the third one popped from $Q$ is $v_2$. $v_2$ is from $\pknnalgpro(v_8)$, $v_1$ is pushed into $Q$ with $dist[v_1] =dist[v_8] + \overline{dist}(v_8,v_1) = 5$. $Q = \{ v_9,v_1| 3,5 \}$, the 4th one from $Q$ is $v_9$. $v_9$ is from $\knnalgpro(v_{20})$,  $v_7$ with $dist[v_7] = dist[v_{20}] + \overline{dist}(v_{20},v_7) = 4$ is pushed into $Q$. Now, $Q = \{v_7, v_1| 4,5 \}$. The 5th from $Q$ is $v_7$. Then the next one from $\knnalgpro(v_{20})$ is $v_8$. Since $v_8$ has been calculated and popped out, we skip this vertex and continue to next one $v_{14}$ with $dist[v_{14}]= dist[v_{20}] + \overline{dist}(v_{20},v_{14}) = 5$. Now $Q = \{v_1, v_{14}| 5,5\}$. The 6th vertex popped from is $v_1$. So the finial computation for $\knnalgpro(v_8) = \{ v_8, v_{20}, v_2, v_9, v_7, v_1\}$ ends.
\end{example}


\begin{theorem}
	The time complexity of \knn$^*$-Index construction is bounded by $O(n \cdot f^2  + n \cdot c \cdot i)$, ($1 \leq i \leq k$, $c = max_{v \in V}|KHV(v)|$).
\end{theorem}

\proofsketch
Refer to \refthm{cutgen}, line 1 needs $O(n \cdot f^2)$. For each vertex, it can be scanned $O(c)$ times, for its $\pknnalgpro$, top $i$ vertices are scanned ($i \leq k$), so the time complexity (lines 5-12) is $O(c \cdot i)$. Similarly, lines 13-27 can be bounded by $O(n \cdot c \cdot i)$. Overall, \knn$^*$-Index construction can be bounded by $O(n \cdot f^2 + n \cdot c \cdot i) (i \leq k)$.
\eop


\subsection{Candidate Object Updates}
\label{sec:update}
Our index contains \knn for all vertices, however, it is unnecessary to update \knn for the whole vertices only due to several objects insertion or deletion. Since some object updates only work for a small part of query vertices, other queries are not affected by these updates. It is unnecessary to be "eager" to update index for all vertices. We adopt a "lazy" update strategy to update index for vertices which are not queried. Especially, we conduct a partial \pknn update strategy. For queries after updating, via the updated \pknn and common updated \knn sharing property, we make a specific index update for the query vertex first, and then return the after-updated and exact \knn for other query vertices.

\subsubsection{\pknn Update for Objects Deletion} The progressive algorithm for deleting a candidate vertex is called \knn$^*$-Delete, and the pseudocode is shown in \refalg{delete}.

First, we record the rank of the deleted vertex $u$ in line 1. In line 2, we only consider the vertex $v$ whose $\pknnalgpro(v)$ contains $u_r$. Similar to the index construction, we update $\pknnalgpro(u_r)$ via $\pknnalgpro(v)$ ($v \in KLV(u_r)$) in line 4. Note that we do not need to recompute  of $\pknnalgpro(v)$. Let $m$ be the new vertex added to $\pknnalgpro(u_r)$. The shortest distance from $m$ to $u_r$ must be not smaller than that from any vertex in the existing $\pknnalgpro(u_r)$ to $u_r$ and not larger than that from any other candidate to $u_r$. Therefore, in lines 5–8, we scan the candidate vertices and derive such vertex $m$. We use a doubly linked list to connect the same vertices in \pknn. Based on the doubly linked list, we efficiently locate the vertices $u_r$ in line 2 of \refalg{delete}. It takes constant time to check whether a vertex belongs to $\pknnalgpro$ of the other vertex.

\begin{algorithm}[htb]
        \caption{\knn$^*$ Delete}
        \label{alg:delete}
        \DontPrintSemicolon            
            \KwInput{$\knnalgpro(\cdot)$ and a deleted vertex $u$}
            \KwOutput{The updated $\pknnalgpro(\cdot)$}
            $r \gets rank(u)$;\;
            \While{$KHV(u_r) \neq \emptyset$ and $u \in \pknnalgpro(u_r)$}{
            delete $u$ from $\pknnalgpro(u_r)$;\;
            $C \gets \bigcup_{v \in KLV(u_r)} \pknnalgpro(v) \setminus \pknnalgpro(u_r)$; \;
            \If{$C \neq \emptyset$}{
            $m \gets argmin_{m \in C}$ $\overline{dist}(m,u_r)$; \;
            $u_r \gets argmin_{u \in KHV(u_r)} rank(u)$; \;
            insert $m$ into the end of $\pknnalgpro(u_r)$; \;
            }
            }
\end{algorithm} 


According to \reflem{pathFirstAndSec}, the maximum number of vertices on the shortest path between any $u$ and $v$ ($u,v \in G$) can be bounded by $l$, we will report $l$ in \refsec{exp}.

\begin{theorem}
	Given the \knn of a graph $G$ and a deleted candidate vertex $u$, the running time of \refalg{delete} is bounded by $O(l \cdot k \cdot p)$, where $p = max_{u \in V} |KLV(u)|$.
\end{theorem}

%\proofsketch
%    The size of $A(u)$ is bounded by $h$. In line 3, the size of XX is XX. Therefore, the total time complexity is $O(h \cdot k \cdot p)$.
%\eop


\subsubsection{Special Query after deleting objects}

\begin{algorithm}[htb]
        \caption{Query after Object Deletion}
        \label{alg:delete_tar}
        \DontPrintSemicolon            
            \KwInput{\knnindex after deleting $u$ and a query vertex $v$}
            \KwOutput{$\knnalgpro(v)$}
            $H \gets \{v\}$;\;
            \While{$KHV(v) \neq \emptyset$}{
            $v \gets argmin_{w\in kHV(v)}rank(w)$;\;
            $H \gets H\cup \{v\}$;\;
            }
            $i \gets |H|-1$;\;
            \While{$i\geq0$ and $KLV(H[i]) \neq \emptyset$ and $u \in \knnalgpro(H[i])$}{
            delete $u$ from $\knnalgpro(H[i])$;\;
            $C \gets (\bigcup_{v \in KHV(H[i])} \knnalgpro(v)) \cup \pknnalgpro(H[i]) \setminus \pknnalgpro(H[i])$; \;
            \If{$C \neq \emptyset$}{
            $m \gets argmin_{m \in C}$ dist($m,H[i]$); \;
            insert $m$ into the end of $\knnalgpro(H[i])$; \;
            }
            $i \gets i-1$; \;
            }
            return $\knnalgpro(v)$;\;
\end{algorithm} 

\begin{theorem}
	Given the partial updated index of a graph $G$ and a deleted candidate vertex $u$, the running time of \refalg{delete_tar} is bounded by $O(l \cdot (k + f))$, where $f = max_{u \in V} |KHV(u)|$.
\end{theorem}

%\proofsketch
%    The size of $A(u)$ is bounded by $h$. In line 3, the size of FV is $f$. Therefore, the total time complexity is $O(h \cdot k \cdot f)$.
%\eop

\subsubsection{Simple Query after Deleting.}
Actually, not all query results after deleting would make big changes. After deleting one object $v_{de}$ from $\mathcal{M}$, there are two situations for a query $\knnalgpro(v_q)$, respectively, $v_{de} \notin \knnalgpro(v_q)$ and $v_{de} \in \knnalgpro(v_q)$. For the first situation $v_{de} \notin \knnalgpro(v_q)$, $\knnalgpro(v_q)$ is the final answer. For the second situation $v_{de} \in \knnalgpro(v_q)$, there are two main cases. We use $v_k$ to represent the $k$th object in the original $\knnalgpro(v_q)$, and use $v_{ik}$ to refer to the $k$th object in the original $\knnalgpro(v_i)$ ($v_i \in KHV(v_q)$). When $v_k \notin V_{ik}$, $V_{ik} = \bigcup_{v_i \in KHV(v_q)}{v_{ik}}$ or $v_k \notin V_{ik}$, $V_{ik} = \bigcup_{v_i \in KHV(v_q)}{v_{ik}}$ and $dist(v_k,v_{ik}) \neq dist(v_k,v_{i}) + dist(v_i,v_{ik})$, we directly scan all $\knnalgpro(v_i)$ ($v_i \in KHV(v_q)$) and skip $v_d$ to calculate updated $\knnalgpro(v_q)$. Otherwise, when $v_k \in V_{ik}$, $V_{ik} = \bigcup_{v_i \in KHV(v_q)}{v_{ik}}$ and $dist(v_k,v_{ik}) = dist(v_k,v_{i}) + dist(v_i,v_{ik})$, we need to update $\knnalg(v_i)$ first. In this situation, the worst case is to start from scratch. However, in practice, the worst case never happens.


\subsubsection{Candidate vertex Insertion}The insertion algorithm is called \knn$^*$-insert, shown as \refalg{insert}.


\begin{algorithm}[htb]
        \caption{\knn$^*$ Insert}
        \label{alg:insert}
        \DontPrintSemicolon            
            \KwInput{\knnindex and a inserted vertex $u$}
            \KwOutput{The updated \knnindex}
            $r \gets rank(u)$; $dist(\cdot) \gets +\infty$;  \; 
            \While{$KHV(u_r) \neq \emptyset$ and $u \notin \pknnalgpro(u_r)$}{
            \For{$w \in KHV(u_r)$}{
            $dist[w] \gets min \{dist[u_r] + dist(u_r,w), dist[w]\};$\;
            }
            $v \gets$ the last vertex in $\pknnalgpro(u_r)$;\;
            \If{$dist(u_r,v) > dist[u_r]$}{
            remove $v$ and insert $u$ into $\pknnalgpro(u_r)$; \;
               }
            $u_r \gets argmin_{w \in KHV(u_r)}rank(w);$\;
            }
\end{algorithm} 

\begin{theorem}
	Given \knn of a graph $G$ and an inserted candidate vertex $u$, the running time of \refalg{insert} is bounded by $O(l \cdot k \cdot p)$.
\end{theorem}


\subsubsection{Targeted-Index Update for Specific Queries.}

\begin{algorithm}[htb]
        \caption{Query after Object Insertion}
        \label{alg:insert_tar}
        \DontPrintSemicolon            
            \KwInput{\knn  after inserting $u$ and a query vertex $v$}
            \KwOutput{$\knnalgpro(v)$}
            $H \gets \emptyset$; $dist(\cdot) \gets +\infty$;\;
            \While{$KHV(v) \neq \emptyset$}{
            $H \gets H\cup \{v\}$;\;
            \For{$w \in KHV(v)$}{
            $dist[w] \gets min \{dist[v] + dist(v,w), dist[w]\};$\;
            }
            $v \gets argmin_{w\in KHV(v)}rank(w)$;\;
            }
            $i \gets |H|-1$;\;
            \While{$i \geq 0$ and $KLV(H[i]) \neq \emptyset$ and $u \notin \knnalgpro(H[i])$}{
            $v_k \gets$ the last vertex in $\knnalgpro(H[i])$;\;
            \If{$dist(H[i],v_k) > dist(H[i],u)$}{
                remove $v$ and insert $u$ into $\knnalgpro(H[i])$; \;
               }
            }
            return $\knnalgpro(H[0])$;\;
\end{algorithm} 

\begin{theorem}
	Given \knnindex of a graph $G$ and an inserted candidate vertex $u$, the running time of \refalg{insert_tar} is bounded by $O(l \cdot k \cdot f)$.
\end{theorem}

\subsubsection{Simple Query after Inserting.}

When answering a query after inserting an object into the candidate set $\mathcal{M}$, it is unnecessary to update \knn for vertices with higher rank than $v_q$, since many them are not queried. In \refsec{exp}, we will show the frequency that vertices can reuse updated \knn, which is very low. So we can skip the step of updating \knn for vertices with higher ranks than $v_q$, which means we only update $\knnalg(v_q)$. To update exact and accurate \knn, we need to calculate the global shortest distance between $v_q$ and $v_{in}$ and then to compare $dist(v_q,v_{in})$ with $dist(v_q,v_k)$ from original $knnalg(v_q)$. Only when $dist(v_q,v_{in}) < dist(v_q,v_k)$, we need to insert $v_{in}$ to an accurate position of $\knnalg(v_q)$ and then delete the final one vertex. Otherwise, $\knnalg(v_q)$ is the answer after updating.
 



==> exp_old.tex <==
\section{Experiments}
\label{sec:exp}

In this section, we compare our algorithms with the state-of-the-art methods for top-k nearest neighbors queries. All experiments are conducted on a machine with an Intel Xeon CPU and 384GB main memory running Linux.

 %an Intel Xeon 2.5GHz CPU (40 cores) and 256 GB main memory running Linux.

\begin{table}[htb]
    {
    %\def\arraystretch{0.9}
    \small{
    \setlength{\tabcolsep}{0.50em}
        \begin{center}
          \begin{tabular}{c| c | r | r | r | r }
            \hline
             \multicolumn{1}{c|}{\cg {Dataset}} & \cg {Name} & \multicolumn{1}{c|}{\cg $n$} & \multicolumn{1}{c|}{\cg $m$} & \multicolumn{1}{c|}{\cg $l$} & \multicolumn{1}{c}{\cg $f$} \\
           \hline
           {New York City} & \kw{NY} & 264,346 & 733,846 & 506 & 134 \\
            \hline
            {San Francisco Bay Area}& \kw{BAY} & 321,270 & 800,172  & 404 & 108 \\
             \hline
            {Colorado} & \kw{COL} & 435,666 & 1,057,066 & 466 & 146 \\
             \hline
            {Florida} & \kw{FLA} & 1,070,376 & 2,712,798 & 521 & 136 \\
             \hline
            {Northwest USA} & \kw{NW} & 1,207,945 & 2,840,208 & 549 & 146 \\ %2,191 
             \hline
            {Northeast USA} & \kw{NE} & 1,524,453 & 3,897,636 & 829 & 219 \\
            \hline
            %\hline
            {California and Nevada} & \kw{CAL} & 1,890,815 & 4,657,742 & 714 & 215 \\
             \hline
            {Great Lakes} & \kw{LKS} & 2,758,119 & 6,885,658 & 1,326  & 370 \\
             \hline
            {Eastern USA} & \kw{EUS} & 3,598,623 & 8,778,114 & 1,023  & 272 \\
             \hline
            {Western USA} & \kw{WUS} & 6,262,104 & 15,248,146 & 1,042 & 326 \\
             \hline
            {Central USA} & \kw{CTR} & 14,081,816 & 34,292,496 & 2,434  & 660 \\
             \hline
            {Full USA} & \kw{USA} & 23,947,347 & 58,333,344 & 2,565  & 693 \\
             \hline
          \end{tabular}
        \end{center}
        }
      }
      \caption{Datasets in experiments}
      \label{tab:dataset}
      \vspace{-0.6cm}
\end{table}
    

\stitle{Datasets.} We use ten publicly available real road networks from DIMACS \footnote{http://users.diag.uniroma1.it/challenge9/download.shtml}. In each road network, vertices represent intersections between roads, edges correspond to roads or road segments, the weight of an edge is the physical distance between two vertices. 
 \reftable{dataset} provides the details about these datasets. \reftable{dataset} shows the value of $l$ and $f$ for each road network and $l$ and $f$ are small in practice. %\reftable{dataset} also shows the value of $\rho$ and $\rho_{\kw{avg}}$ of \lcdpindex for each road network, where $\rho_{\kw{avg}}$ represents the average size of  \kw{LCDS} in \lcdpindex. It is clear that $\rho$ and  $\rho_{\kw{avg}}$ are much smaller than $h$ and $\omega$ in practice.

\stitle{Algorithms.} We compare the following algorithms. All the algorithms are implemented in C++ and compiled in GCC 10.2.1 with -O3 flag. 

\begin{itemize}[leftmargin=*]
	\item \kw{Dijkstra}: A naive method to compute global KNN for all vertices in a given graph $G$.
	\item \kw{TEN-Index}: The state-of-the-art algorithm for KNN queries, which is introduced in \refsec{existing}.
	\item \kw{TEN-KNN}: Calculating KNN for all vertices using TEN-Index.
	\item \kw{UG-KNN}: Our UG-based index construction algorithms (\refsec{ug}).
   \item \kw{UTL-KNN}: Our opitimized algorithms (\refsec{utl}).
\end{itemize}

\stitle{Parameter Settings.} Following previous KNN works\cite{ouyang2020progressive, he2019efficient, luo2018toain}, we randomly select the set of candidate objects in each dataset. The candidate density $\rho$ and the query parameter $k$ settings are shown in \reftable{para}, default values display in bold and Italic font. Here, density $\rho$, the result of dividing the size of candidate object set $\mathcal{M}$ into the size of the whole vertices $V$ in the dataset, formally, $\rho = |\mathcal{M}|/|V|$.

\begin{table}[htb]
    {
    %\def\arraystretch{0.9}    
    \setlength{\tabcolsep}{0.55em}
        \begin{center}
          \begin{tabular}{c| c }
            \hline
             \multicolumn{1}{c|}{\cg {Parameters}} & \multicolumn{1}{c}{\cg Values}\\
           \hline
           {$\rho$} & {0.5, 0.1, 0.05, 0.01, \emph{\textbf{0.005}}, 0.001, 0.0005, 0.0001}\\
            \hline
            {$k$}& {2,000, 1,000, 500, 200, 100, \emph{\textbf{40}}, 20 }\\
            \hline
          \end{tabular}
        \end{center}
        }
      \caption{Parameter Settings}
      \label{tab:para}
      \vspace{-0.6cm}
\end{table}

\begin{figure*}[tb]
  \centering
 %\hspace{-0.1cm}\incluegraphics[width = 1\linewidth]{exp/IndexSize.pdf}
 \hspace{-0.5cm}\includegraphics[width=0.95\linewidth]{exp/KnnIndexSize.pdf}
  \caption{Index Size Comparison (MB)}
  \label{fig:indexsize}
   %\vspace{-0.3cm}
\end{figure*}

\begin{figure*}[htb]
  \centering
 %\hspace{-0.1cm}\incluegraphics[width = 1\linewidth]{exp/IndexSize.pdf}
 \hspace{-0.5cm}\includegraphics[width=0.55\linewidth]{exp/tuli.jpg}
  %\caption{Indexing Time Comparison (s)}
  \label{fig:indextime}
   \vspace{-1cm}
\end{figure*}

\begin{figure*}[htb]
  \centering
 %\hspace{-0.1cm}\incluegraphics[width = 1\linewidth]{exp/IndexSize.pdf}
 \hspace{-0.5cm}\includegraphics[width=0.95\linewidth]{exp/KnnIndexTime.pdf}
  \caption{Indexing Time Comparison (s)}
  \label{fig:indextime}
   %\vspace{-0.3cm}
\end{figure*}


\begin{figure*}[htb]
  \centering
  \subfigcapskip=0pt
  \subfigure[NY]{\includegraphics[width=0.19\linewidth]{exp/NY_dq.pdf}}\label{fig:nyqvden}
  %\subfigure[BAY]{\includegraphics[width=0.16\linewidth]{exp/BAY_dq.pdf}}\label{fig:bayqvden}
  \subfigure[COL]{\includegraphics[width=0.19\linewidth]{exp/COL_dq.pdf}}\label{fig:colqvden}
  \subfigure[FLA]{\includegraphics[width=0.19\linewidth]{exp/FLA_dq.pdf}}\label{fig:flaqvden}
  \subfigure[NW]{\includegraphics[width=0.19\linewidth]{exp/NW_dq.pdf}}\label{fig:nwqvden}
  \subfigure[NE]{\includegraphics[width=0.19\linewidth]{exp/NE_dq.pdf}}\label{fig:neqvden}\\
  \subfigure[CAL]{\includegraphics[width=0.19\linewidth]{exp/CAL_dq.pdf}}\label{fig:calqvden}
  %\subfigure[LKS]{\includegraphics[width=0.16\linewidth]{exp/LKS_dq.pdf}}\label{fig:lksqvden}
  \subfigure[EUS]{\includegraphics[width=0.19\linewidth]{exp/E_dq.pdf}}\label{fig:eqvden}
  \subfigure[WUS]{\includegraphics[width=0.19\linewidth]{exp/W_dq.pdf}}\label{fig:wqvden}
  \subfigure[CTR]{\includegraphics[width=0.19\linewidth]{exp/CTR_dq.pdf}}\label{fig:ctrsqden}
  \subfigure[USA]{\includegraphics[width=0.19\linewidth]{exp/USA_dq.pdf}}\label{fig:usasqden}\\
     %\vspace{-0.5cm}
  \caption{Query Processing time Varys with different Density $\rho$}
  \label{fig:queryvd}
   %\vspace{-0.3cm}
\end{figure*}


\begin{figure*}[htb]
  \centering
  \subfigcapskip=0pt
  \subfigure[NY]{\includegraphics[width=0.19\linewidth]{exp/NY_vk.pdf}}\label{fig:nyqvk}
  %\subfigure[BAY]{\includegraphics[width=0.16\linewidth]{exp/BAY_vk.pdf}}\label{fig:bayqvk}
  \subfigure[COL]{\includegraphics[width=0.19\linewidth]{exp/COL_vk.pdf}}\label{fig:colqvk}
  \subfigure[FLA]{\includegraphics[width=0.19\linewidth]{exp/FLA_vk.pdf}}\label{fig:flaqvk}
  \subfigure[NW]{\includegraphics[width=0.19\linewidth]{exp/NW_vk.pdf}}\label{fig:nwqvk}
  \subfigure[NE]{\includegraphics[width=0.19\linewidth]{exp/NE_vk.pdf}}\label{fig:neqvk}\\
  \subfigure[CAL]{\includegraphics[width=0.19\linewidth]{exp/CAL_vk.pdf}}\label{fig:calqvk}
  %\subfigure[LKS]{\includegraphics[width=0.16\linewidth]{exp/LKS_vk.pdf}}\label{fig:lksqvk}
  \subfigure[EUS]{\includegraphics[width=0.19\linewidth]{exp/E_vk.pdf}}\label{fig:eqvk}
  \subfigure[WUS]{\includegraphics[width=0.19\linewidth]{exp/W_vk.pdf}}\label{fig:wqvk}
  \subfigure[CTR]{\includegraphics[width=0.19\linewidth]{exp/CTR_vk.pdf}}\label{fig:ctrqvk}
  \subfigure[USA]{\includegraphics[width=0.19\linewidth]{exp/USA_vk.pdf}}\label{fig:usaqvk}\\
     %\vspace{-0.5cm}
  \caption{Query processing time Varys with different $k$}
  \label{fig:queryvk}
   %\vspace{-0.3cm}
\end{figure*}



\stitle{Exp-1: Index Size Comparison} \reffig{indexsize} shows the index size of UTL-KNN, TEN-Index. Since both Dijkstra and KNN-TEN compute top k nearest neighbors for all vertices in graph, their finial index size are both same with our KNN$^*$-Index. We do not show their index size repetitively. As shown in \reffig{indexsize}, the index space of KNN$^*$-Index is much smaller than that of TEN-Index. Specifically, for $USA$, the index size of KNN$^*$-Index is smaller 44 times than the size of TEN-Index. TEN-Index size is $167.1$ GB. However, our KNN$^*$-Index size is only $3.9$ GB. The results verify the effectiveness of KNN$^*$-Index on reducing the index space.

%TOAIN uses the smallest space because it is based on Contraction Hierarchies. It costs 93MB for NY and 1, 862MB for E-US. GLAD uses too much memory space and the index for US cannot be successfully constructed in the experiment machine with 256 GB RAM. GLAD consumes 521 MB for NY and 136, 315MB for CTR. TEN$^*$-Construct uses 466 MB for NY and 101,967 MB for CTR, respectively.

%For example, the indexing time of \ctspc 115.98 times less than that of \hpspc on \kw{DB}. Moreover, \hpspc cannot finish the index construction for \kw{ST}, \kw{SN}, \kw{IT}, and \kw{SK} in the set time, while \ctspc finishes the index construction for all these datasets in a reasonable time. %For example, for the largest dataset \kw{SK}, \ctspc finishes the index construction in 23,059 seconds. 

\stitle{Exp-2: Indexing Time Comparison} \reffig{indextime} shows the indexing time of \knn$^*$-Index, TEN-Index, Dijkstra and TEN-KNN. As shown in  \reffig{indextime}, the indexing time of \knn$^*$-Index is significantly less than that of TEN-Index. Indexing time of \knn$^*$-Index is the fastest in all datasets, which takes 248 seconds for USA. However, even though TEN-Index computes partial KNN index, the indexing time of TEN-Index still needs $19666.157$s, which contains H2H-Index construction time $19632.1$s. The indexing time of TEN-KNN and that of TEN-Index are similar, since TEN-KNN is based on the TEN-Index which also use the huge H2H-Index.

\stitle{Exp-3: Query Processing Time with Varying Density $\rho$.} We randomly generate $10,000$ queries for every dataset and for every density $\rho$. We report the average processing time for each query with $k = 200$. \reffig{queryvd} shows the query processing time of \tenindex and \knnindex when varying $\rho$. With the decrease of the density of object set, the query delay of \tenindex grows more intensively than that of \knnindex. Especially, the speedup from \tenindex to \knnindex is up to 3 orders in CTR dataset when $\rho = 0.0001$. The more sparsely the object set distributes, better the query speedup performance is.


\stitle{Exp-4: Query Processing Time with Varying $k$.} We randomly generate $10,000$ queries for every dataset and for each $k$ with $\rho = 0.005$. We report the average processing time for each query. We report our query result with different $k$ in \reffig{queryvk}. Obviously, with increase of $k$, the growth of query processing delay of \tenindex is faster than the increase for our \knnindex's query delay.

%\stitle{Exp-5: Indexing Time Comparison between \knnindex and \knn$^*$-Index.} As complexity analysis in \refsec{naive} and \refsec{pro}, we compare the indexing time for \knnindex and \knn$^*$-Index in \reftable{com_idxtime}. Here, the indexing time only denotes the \knn construction time, which does not contain the vertex cut generation time, since the time for generating vertex cut is the same. To compare the indexing time directly, we only compare \knn computation time. Although the speedup between \knnindex and \knn$^*$-Index is not so huge for the whole graph, the index update based on \knn$^*$-Index for some vertices deletion or insertion is obvious, we will show this in Exp-7.

\begin{table}[htb]
    {
    %\def\arraystretch{0.9}    
    \setlength{\tabcolsep}{0.55em}
        \begin{center}
          \begin{tabular}{c  c  c  c  c  c  c }
            \hline
             \multicolumn{1}{c}{ { }} & \multicolumn{1}{c}{ NY} & \multicolumn{1}{c}{ COL} & \multicolumn{1}{c}{ FLA} & \multicolumn{1}{c}{ NW} & \multicolumn{1}{c}{ NE}\\
           \hline
           {$\knn$} & 4.65 & 6.18 & 15.45 & 16.71 & 25.24\\
            \hline
            {$\knn^*$} & 3.62 & 4.93 & 12.35 & 13.70 & 19.81\\
            %{$VCT^*$} & 7.05 & 7.10 & 9.25 & 23.06 & 24.92 & 37.57\\
            \hline
            \multicolumn{1}{c}{ {}} & \multicolumn{1}{c}{ CAL} & \multicolumn{1}{c}{ EUS} & \multicolumn{1}{c}{ WUS} & \multicolumn{1}{c}{ CTR} & \multicolumn{1}{c}{ USA}\\
           \hline
           {$\knn$} & 28.08 & 54.67 & 91.99 & 236.51 & 379.76\\
            \hline
            {$\knn^*$} & 22.28 & 43.80 & 73.66 & 182.70 & 299.68\\            %{$VCT^*$} & 42.29 & 72.81 & 83.83 & 140.62 & 386.57 & 602.48\\
            \hline
          \end{tabular}
        \end{center}
    }
       \caption{Indexing Time(s) for $\knn$ and $\knn^*$}
      \label{tab:com_idxtime}
      \vspace{-0.6cm}
\end{table}

In \reftable{com_ave_cand_size}, we report the average number of candidate objects for constructing \knnindex and \knn$^*$-Index under the $k=200$ and $\rho = 0.005$ setting. To compare clearly, the size of candidate set $|\mathcal{M}|$ is shown in the first level. From \reftable{com_ave_cand_size}, we can see that the explored candidate objects is significantly pruned for computing \knn.

\begin{table}[htb]
    {
    %\def\arraystretch{0.9}    
    \setlength{\tabcolsep}{0.55em}
        \begin{center}
          \begin{tabular}{c  c  c  c  c  c  c }
            \hline
             \multicolumn{1}{c}{ { }} & \multicolumn{1}{c}{ NY} &  \multicolumn{1}{c}{ COL} & \multicolumn{1}{c}{ FLA} & \multicolumn{1}{c}{ NW} & \multicolumn{1}{c}{ NE}\\
           \hline
           {$|\mathcal{M}|$} & 1,321  & 2,178 & 5,351 & 6,039 & 7,622\\
            \hline
            {$\knn$} & 0.737 & 0.273 & 0.117 & 0.091 & 0.099\\
            %{$VCT$} & 0.156 & 0.127 & 0.094 & 0.038 & 0.034 & 0.027\\
            \hline
            {$\knn^*$} & 0.153& 0.092 & 0.038 & 0.033 & 0.026\\
            \hline
            \multicolumn{1}{c}{ {}} & \multicolumn{1}{c}{ CAL} & \multicolumn{1}{c}{ EUS} & \multicolumn{1}{c}{ WUS} & \multicolumn{1}{c}{ CTR} & \multicolumn{1}{c}{ USA}\\
           \hline
           {$|\mathcal{M}|$} & 9,454 & 17,993 & 31,310 & 70,409 & 119,736\\
           \hline
           {$\knn$} & 0.068 & 0.036 & 0.020 & 0.010 & 0.006\\
           %{$VCT$} & 0.022 & 0.015 & 0.011 & 0.007 & 0.003 & 0.002\\
            \hline
            {$\knn^*$} & 0.021 & 0.011 & 0.006 & 0.003 & 0.002\\
            \hline
          \end{tabular}
        \end{center}
    }
       \caption{Average Candidate Size for $\knn$ and $\knn^*$}
      \label{tab:com_ave_cand_size}
      \vspace{-0.6cm}
\end{table}


\stitle{Exp-6: \knnindex size varies with different $k$ and $\rho$.} %One basic reason for performance promotion from \knnindex (in \refsec{naive}) to \knn$^*$-Index(in \refsec{pro}) is the vertex cut extraction. Here, we denote $VC(\cdot) = LV(\cdot) \cup HV(\cdot)$ and $KVC(\cdot) = KLV(\cdot) \cup KHV(\cdot)$. We report the sum size of $VC$ and $KVC$ for the whole vertices in \reftable{comp_vc_kvc}. For NY, the vertex cut size is reduced by 315,808, compared with the original vertex cut. For USA, the size of key vertex cut $|KVC|$ is decreased by $17,020,287$. This vertex cut extraction helps more in the lazy update in Exp-7.
%\begin{table}[htb]
%    {   
%    \setlength{\tabcolsep}{0.35em}
%        \begin{center}
%          \begin{tabular}{c  c  c  c  c  c  c }
%            \hline
%             \multicolumn{1}{c}{ { }} & \multicolumn{1}{c}{ NY} &  \multicolumn{1}{c}{ COL} & \multicolumn{1}{c}{ FLA} & \multicolumn{1}{c}{ NW} & \multicolumn{1}{c}{ NE}\\
%           \hline
%           {$VC$} & 1,286,136  & 1,295,817 & 3,355,280 & 3,311,040 & 5,741,496\\
%            \hline
%            {$KVC$} & 970,328  & 1,092,602 & 2,840,826 & 2,840,282 & 4,556,471\\
%            \hline
%            \multicolumn{1}{c}{ {}} & \multicolumn{1}{c}{ CAL} & \multicolumn{1}{c}{ EUS} & \multicolumn{1}{c}{ WUS} & \multicolumn{1}{c}{ CTR} & \multicolumn{1}{c}{ USA}\\
%           \hline
%           {$VC$} & 6,097,173 & 11,695,085 & 19,604,543 & 49,338,558 & 81,695,081\\
%            \hline
%            {$KVC$} & 5,030,155 & 9,577,052 & 16,265,769 & 38,473,060 & 64,674,794\\
%            \hline
%          \end{tabular}
%        \end{center}
%    }
%       \caption{ Comparison between $VC$ and $KVC$ }
%      \label{tab:comp_vc_kvc}
%      \vspace{-0.6cm}
%\end{table}

\stitle{Exp-6: \knnindex indexing time varies with different $k$ and $\rho$.}

\stitle{Exp-7: Object Update.}
We evaluate our lazy update algorithms and special targeted query algorithms in experiments. To generate update queries, we randomly select a vertex u and an operation (either insertion or deletion). We skip the query if $u \in \mathcal{M}$ for insertion and $u \in \mathcal{M}$ for deletion. For each dataset, we repeat this step until 10, 000 updates are generated. The average time for each update operation is reported in \reffig{up_in}. \knn$^*$-Index uses \refalg{delete} and \refalg{insert} for objects deletion and objects insertion in \refsec{pro}, and \knn-Index uses the algorithm mentioned in \refsec{naive} for objects deletion. \knn$^*$-Update is lightly slower than \tenindex. For the targeted queries, even if our queries are slower than \tenindex, our simple queries are still faster than \tenindex.


\begin{figure}[htb]
 \vspace{-0.1cm}
  \centering
   \subfigcapskip=0pt
   \subfigcaptopadj=0pt
   \includegraphics[width=0.95\linewidth]{exp/knnUpdate_in.pdf}
  \vspace{-0.1cm}
 \caption{Update Time for Insert (s)}
  \label{fig:up_in}
  \vspace{-0.1cm}
\end{figure}

\begin{figure}[htb]
 \vspace{-0.1cm}
  \centering
   \subfigcapskip=0pt
   \subfigcaptopadj=0pt
   \includegraphics[width=0.95\linewidth]{exp/knnUpdate_de.pdf}
  \vspace{-0.1cm}
 \caption{Update Time for Delete (s)}
  \label{fig:up_de}
  \vspace{-0.1cm}
\end{figure}


%\begin{figure}[htb]
% \vspace{-0.1cm}
%  \centering
%   \subfigcapskip=0pt
%   \subfigcaptopadj=0pt
%   \subfigure[Update for Insert(s)]{ \includegraphics[width=0.45\linewidth]{exp/KnnUpdate_in.pdf}}
% \subfigure[Update for Delete(s)]{ \includegraphics[width=0.45\linewidth]{exp/KnnUpdate_de.pdf}}
%  \vspace{-0.1cm}
%  \caption{Update Time for Insert (s)}
%  \label{fig:up_in}
%  \vspace{-0.1cm}
%\end{figure}


\begin{figure}[htb]
 \vspace{-0.1cm}
  \centering
   \subfigcapskip=0pt
   \subfigcaptopadj=0pt
   \includegraphics[width=0.95\linewidth]{exp/knnUpdateQ_in.pdf}
  \vspace{-0.1cm}
 \caption{Query Time for Insert (s)}
  \label{fig:qu_in}
  %\vspace{-0.1cm}
\end{figure}

\begin{figure}[htb]
 \vspace{-0.1cm}
  \centering
   \subfigcapskip=0pt
   \subfigcaptopadj=0pt
   \includegraphics[width=0.95\linewidth]{exp/knnUpdateQ_de.pdf}
  \vspace{-0.1cm}
 \caption{Query Time for Delete (s)}
  \label{fig:qu_de}
  %\vspace{-0.1cm}
\end{figure}


\stitle{Exp-8: Scalability when varying graph size.} In this experiment, we evaluate the scalability of \knnindex and \tenindex. To test the scalability for indexing time and index size, we vary the dataset size (the number of vertices in the road networks) from $10^6$ to $24 * 10^6$. We divide the whole US into $10 * 10$ grids on the map and generate ten road networks using the $1*1, 2*2, . . . , 10*10$ grids from the middle of the map. We denote them as $G_1,G_2,...,G_{10}$ respectively. We report the index size and the indexing time in \reffig{sc_size} and \reffig{sc_time}, respectively. When the dataset increases from $10^6$ to $24 * 10^6$, the indexing time increases stably for all algorithms, which verifies our KNN$^*$-Index has a good scalability. Also, compared with \tenindex, our KNN$^*$-Index always outperforms. 

\begin{figure}[htb]
 \vspace{-0.1cm}
  \centering
   \subfigcapskip=0pt
   \subfigcaptopadj=0pt
 \subfigure[Index Size]{ \includegraphics[width=0.45\linewidth]{exp/USA_scal_size.pdf}
     \label{fig:sc_size}}
 \subfigure[Indexing Time]{ \includegraphics[width=0.45\linewidth]{exp/USA_scal_time.pdf}
     \label{fig:sc_time}}
  \vspace{-0.1cm}
 \caption{Scalability Testing}
  \label{fig:scale}
  %\vspace{-0.1cm}
\end{figure}


\stitle{Exp-9: System throughput.}









==> update_old.tex <==
\section{Candidate Object Update}
\label{sec:update}

In some cases, the candidate objects $\mathcal{M}$ may be updated. In this section, we discuss how to maintain the \knnindex when the candidate object are update. Therefore, we adopt an update on-demand a



Our index contains \knn for all vertices. However, it is unnecessary to update \knn for the whole vertices only due to several objects insertion or deletion. Some object updates only work for a small part of query vertices, other queries are not affected by these updates. It is unnecessary to be \stitle{\emph{eager}} to update index for all vertices. We adopt a \stitle{\emph{lazy}} update strategy to update index for vertices which are not queried. Especially, we conduct a partial update strategy, which updates $\pknnalg(\cdot)$ first. For queries after updating, via the updated $\pknnalg(\cdot)$, we make a correspond $\knnalg(\cdot)$ update for the query vertex. 


\subsection{Object Deletion}

\stitle{Update $\pknnalg(v), v \in \sdgu(u)$.} The algorithm for deleting a candidate object $u$ is called $\kw{KNN}\textrm{-}\kw{Index}\textrm{-}\kw{Delete^+}(G, \pknnalg(\cdot), u)$, and the pseudocode is shown in \refalg{delete}.

We construct $\sdgu(u)$ for a deleted object $u$ (line 1) and iterate every vertex $v \in V(\sdgu(u))$ in the increasing order of $\pi(v)$ (line 2). If $\pknnalg(v)$ does not contain $u$, we directly go to the next vertex in $\sdgu(u)$ (line 3-4). Otherwise, we delete $u$ from $\pknnalg(v)$ (line 5). Similar to the $\pknnalg(\cdot)$ construction, we update $\pknnalg(u_i)$ via constructing $\mathcal{S}$ from $\cup_{w \in \keyL(v)}\pknnalg(w) \setminus \pknnalg(v)$ (line 6). When $\mathcal{S}$ is not an empty set, we insert the vertex $v$ with the smallest decreasing rank distance in $\mathcal{S}$ into the end of $\pknnalg(v)$ (line 7-9). 


%First, we record the rank $\pi(u)$ of the deleted vertex $u$ in line 1. In line 2, we only consider the vertex $v$ whose $\pknnalg(v)$ contains $u_d$. Similar to the index construction, we update $\pknnalg(u_i)$ via $\pknnalg(w)$ ($w \in \keyL(u_i)$) in line 4. Note that we do not need to recompute  of $\pknnalg(w)$. Let $m$ be the new vertex added to $\pknnalg(u_i)$. The shortest distance from $m$ to $u_i$ must be not smaller than that from any vertex in the existing $\pknnalg(u_i)$ to $u_i$ and not larger than that from any other candidate to $u_i$. Therefore, in lines 5–8, we scan the candidate vertices and derive such vertex $v$. We use a doubly linked list to connect the same vertices in \pknn. Based on the doubly linked list, we efficiently locate the vertices $u_i$ in line 2 of \refalg{delete}. It takes constant time to check whether a vertex belongs to $\pknnalg$ of the other vertex.

\begin{algorithm}[htb]
        \caption{$\kw{KNN}\textrm{-}\kw{Index}\textrm{-}\kw{Del}(G, G', \pknnalg(\cdot), u)$}
        \label{alg:delete}
        \small
        \DontPrintSemicolon            
            %\KwInput{$\knnalg(\cdot)$ and a deleted vertex $u$}
            %\KwOutput{The updated $\pknnalg(\cdot)$}
            construct $\sdgu(u)$ by conducting BFS search from $u$ on $G'$ following $edge(v,v')$ with $\pi(v)<\pi(v')$;\;
            	\For{\textbf{each} $v \in V(\sdgu(u))$ in increasing order of $\pi(v)$}{
           		\If{$u \notin \pknnalg(v)$}{continue;}
           		delete $u$ from $\pknnalg(v)$;\;
            		$\mathcal{S} \gets \cup_{w \in \keyL(v)} \pknnalg(w) \setminus \pknnalg(v)$;\;
            		\If{$\mathcal{S} \neq \emptyset$}{
            			$m \gets argmin_{m \in \mathcal{S}}  \psd(m,v)$;\;
            			insert $m$ into the end of $\pknnalg(v)$;\;
            		}
            }
\end{algorithm} 


\begin{theorem}
	Given the \sdg $G'$ and $\pknnalg(\cdot)$ of a graph $G$, and a deleted  object $u$, the time complexity of \refalg{delete} is bounded by $O(\eta \cdot k \cdot \tau)$, where $\eta = \kw{max}_{v \in V(G)}|\sdgu(v)|$ and $\tau = max_{v \in V(G)} |\keyU(v)|$.
\end{theorem}

\proofsketch
	 We need $O(\eta \cdot \tau)$ to construct $\sdgu(u)$ using BFS (line 1). Since  $\pknnalg(v)$ is stored in a doubly linked list, it takes $O(k)$ to check whether $u$ is in $\pknnalg(v)$ (line 3). In line 6, each vertex $w$ is only iterated by its $\keyU(w)$ and $|\pknnalg(w)| \leq k$. So the time complexity is $O(\eta \cdot (k + k \cdot \tau)) = O(\eta \cdot k \cdot \tau)$ (line 2-9). Therefore, the total time complexity of \refalg{delete} is $O(\eta \cdot \tau + \eta \cdot k \cdot \tau) = O(\eta \cdot k \cdot \tau)$.
\eop

The first part $O(\eta)$ in the time complexity can be very small in practice, since we only need to process the vertex $v \in V(\sdgu(u))$ that $u \in \pknnalg(v)$.

\stitle{\knnindex Update.} The algorithm for $q$'s $k$NN query after deleting an object $u$ is shown in \refalg{delete_tar}.

There are four cases for answering $k$NN query of a vertex $q$ after deleting an object $u$. (1) when $u \notin \knnalg(q)$, the original $\knnalg(q)$ is the answer (line 1-2). Before introducing case 2, we first denote the last one from $\knnalg(w), w \in \keyU(q)$ as $w_k$. We collect them into $\mathcal{S}_k$, i.e., $\mathcal{S}_k = \{w_k |$ the last one vertex $w_k \in \knnalg(w), \forall w \in \keyU(u)\}$. And we also record the upper bound of distance as $d$ (line 3-7). (2) When $u \notin \mathcal{S}_k$ and $u \neq q_k$, we first remove $u$ from $\knnalg(q)$ (line 10). Then, we construct $\mathcal{S} = \cup_{w \in \keyU(q)}\knnalg(w) \cup \pknnalg(q) \setminus \knnalg(q)$ (line 11). We insert the vertex $m$ with smallest distance from $\mathcal{S}$ to $\knnalg(q)$, then return  the answer (line 12-15). (3) When $u \in \mathcal{S}_k$ or $u = q_k$, but $\sd((u,q),G) \neq d$ and $\sd((u,q),G) \neq d_k$, we return the answer in the same way as case 2 (line 16). (4) When $u \in \mathcal{S}_k$ or $u = v_k$, and $\sd((u,q),G) = d$ or $\sd((u,q),G) = d_k$, we first construct $\sdgu(q)$ for the query vertex $q$ (line 17) and iterate every vertex $v \in V(\sdgu(q))$ in the decreasing order of $\pi(v)$ (line 18). If $\pknnalg(v)$ does not contain $u$, we directly go to the next vertex in $\sdgu(q)$ (line 19-20). Otherwise, we delete $u$ from $\pknnalg(v)$ (line 21). Similar to the $\knnalg(\cdot)$ construction, we update $\knnalg(v)$ via $\mathcal{S} = \cup_{w \in \keyU(v)}\knnalg(w) \cup \pknnalg(v) \setminus \knnalg(v)$ (line 22). When $\mathcal{S}$ is not an empty set, we insert the vertex $m$ with smallest distance from $\mathcal{S}$ into the end of $\knnalg(v)$ (line 23-25).

\begin{algorithm}[htb]
        %\caption{$\kw{KNN^*}\textrm{-}\kw{Index}\textrm{-}\kw{Delete}(G, \pknnalg(\cdot), u)$}
        %\caption{$\kw{KNN}\textrm{-}\kw{Index}\textrm{-}\kw{Query}\textrm{-}\kw{after}\textrm{-}\kw{Delete^*}(G', \pknnalg(\cdot), u)$}
        \caption{$\kw{KNN}\textrm{-}\kw{Index}\textrm{-}\kw{Del}(G, G', \pknnalg(\cdot), \knnalg(\cdot), u, q)$}
        \small
        \label{alg:delete_tar}
        \DontPrintSemicolon            
            %\KwInput{\knnindex after deleting $u$ and a query vertex $v$}
            %\KwOutput{$\knnalg(v)$}
            	\tcp{Case 1}
            	\If{$u \notin \knnalg(q)$}{ return $\knnalg(q)$;}
            	$\mathcal{S}_k \gets \emptyset$; $d \gets +\infty$;\;
            	\For{$w \in \keyU(q)$}{
            		$w_k \gets$ the last one vertex in $\knnalg(w)$;  \; 
            		$\mathcal{S}_k \gets \mathcal{S}_k \cup \{w_k\}$; \;
            		$d \gets \min\{\phi((q,w),G') + \sd((w,w_k),G), d\}$; \;
            	}
            	$q_k \gets $ the last one in $\pknnalg(q)$; $d_k \gets \psd(q,q_k)$;\;
            	\tcp{Case 2}
            	\If{$u \notin \mathcal{S}_k$ and $u \neq v_k$}{
            		delete $u$ from $\knnalg(q)$; \;
            		$\mathcal{S} \gets \cup_{w \in \keyU(q)} \knnalg(w) \cup \pknnalg(q) \setminus \knnalg(q)$; \;
            		\If{$\mathcal{S} \neq \emptyset$}{
            			$m \gets argmin_{m \in \mathcal{S}} \sd(m,q)$; \;
            			insert $m$ into the end of $\knnalg(q)$; \;
            			return $\knnalg(q)$;
            		}
            	}
            	\tcp{Case 3}
            	\ElseIf{$(\sd((u,q),G) \neq d$ and $\sd((u,q),G) \neq d_k$}{
            	\tcp{same procedure with Case 2 (line 10-15).}
            	}
            %\tcp{Case 3}
            	%\ElseIf{$\sd(u,v) \neq d$}{
            		%$\mathcal{S} \gets \cup_{w \in \keyU(v)} \knnalg(w) \cup \pknnalg(u) \setminus \knnalg(u)$; \;
            			%\If{$\mathcal{S} \neq \emptyset$}{
            				%$m \gets argmin_{m \in \mathcal{S}} \sd(m,u)$; \;
            				%insert $m$ into the end of $\knnalg(u)$; \;
            				%return $\knnalg(u)$;
            			%}
           %}
            	\tcp{Case 4}
            construct $\sdgu(q)$ by conducting BFS search from $q$ on $G'$ following $edge(v,v')$ with $\pi(v)<\pi(v')$;\;
            	\For{\textbf{each} $v \in V(\sdgu(q))$ in decreasing order of $\pi(v)$}{
            		\If{$u \notin \knnalg(v)$}{continue;}
            		delete $u$ from $\knnalg(v)$; \;
            		$\mathcal{S} \gets \cup_{w \in \keyU(v)} \knnalg(w) \cup \pknnalg(v) \setminus \knnalg(v)$; \;
            		\If{$\mathcal{S} \neq \emptyset$}{
            			$m \gets argmin_{m \in \mathcal{S}} \sd(m, v)$; \;
            			insert $m$ into the end of $\knnalg(v)$; \;
            		}
            }
            return $\knnalg(q)$;\;
\end{algorithm} 

\begin{theorem}
	Given the \sdg $G'$ of the graph $G$, updated $\pknnalg(\cdot)$, a deleted object $u$ and a query vertex $q$, the time complexity of \refalg{delete_tar} is $O(\eta \cdot k \cdot \tau)$, where $\eta = \kw{max}_{v \in V(G)}|\sdgu(v)|$ and $\tau = \kw{max}_{v \in V(G)}|\keyU(v)|$.
\end{theorem}

\proofsketch
	Since $\knnalg(q)$ is stored in a doubly linked list, we need $O(k)$ for checking whether $u$ is in $\knnalg(q)$ (line 1-2). We can obtain $\mathcal{S}_k$ and $d$ in $O(\tau)$. We can update $\knnalg(v)$ in $O(\tau \cdot k)$ for case 2 or 3 (line 10-15). For the case 4, the size of $\mathcal{S}$ is bounded by $|\mathcal{S}| = (|\keyU(v)| + 1) \cdot |\knnalg(w)| \leq (\tau+1) \cdot k \leq \tau \cdot k$ (line 22). Therefore, the total time complexity of \refalg{delete_tar} is $O(\eta \cdot k \cdot \tau)$.
\eop

%When there are many queries after deletes, the first part in the time complexity $O(\eta)$ is small in practice, since the upper graphs for these queries may exist intersections, in which the vertices do not need to be updated again. Especially, when the query vertex $u$ belongs to someone query vertex's upper graph, $\knnalg(u)$ can directly be returned as the final answer.

%Actually, not all query results after deleting some candidate objects would be affected. After deleting one object $v_{de}$ from $\mathcal{M}$, there are two situations for a query $\knnalg(v_q)$, respectively, $v_{de} \notin \knnalg(v_q)$ and $v_{de} \in \knnalg(v_q)$. For the first situation $v_{de} \notin \knnalg(v_q)$, the original $\knnalg(v_q)$ is the final answer after deleting objects. For the second situation $v_{de} \in \knnalg(v_q)$, there are three subcases. We use $v_k$ to represent the $k$th object in the original $\knnalg(v_q)$, and use $w_{k}$ to refer to the $k$th object in the original $\knnalg(w)$ ($w \in \keyU(v_q)$). We collect all $w_k$ for all $w \in \keyU(v_q)$ as $U_k$, i.e., $U_k = \cup_{w \in \keyU(v_q)}\{ w_k \}$. For the first subcase, $v_{de} \notin U_k$, we directly scan all $\knnalg(w)$ ($w \in \keyU(v_q)$) and skip $v_{de}$ to calculate updated $\knnalg(v_q)$. For the second subcase, $v_{de} \in U_k$ and $v_{de} = w_k$ from $\knnalg(w)$, but $\sd(v_q,v_{de}) \neq \sd(v_q,w) + \sd(w, w_k)$, which denotes that even if $v_{de} \in U_k$ but $v_{de}$ in someone $\knnalg(w)$ is not the final one, we still can use the solution for the first subcase. Otherwise, when $v_{de} \in U_k$ and there is a vertex $w \in \keyU(v_q)$ such that $dist(v_q, w_k) = dist(v_q,w) + dist(w,w_k)$, we need to update $\knnalg(w)$ first. In this situation, the worst case is to start from scratch. However, in practice, the worst case happens occasionally.


\subsection{Object Insertion} 

When an object is inserted in the. We follow the. The two algorithms are shows in  \refalg{} and \refalg{}, respectively.


\stitle{.}

The algorithm for inserting a candidate object $u$ is shown in \refalg{insert}.

\refalg{insert} shows the procedure of collecting $V(\sdgu(u))$ for the inserted object $u$ and calculate the decreasing rank distance between $u$ and each vertex $v$ in $V(\sdgu(u)$, i.e, $\psd(u,v)$, for $v \in V(\sdgu(u))$, which is stored in the array $\psd[u,\cdot]$. We first initialize $v, V(\sdgu(u)),$ and $\psd[u,\cdot]$ (line 1-2). According to \refdef{lg}, we only need to explore the vertex $w$ in $\keyU(v)$. Referring to \refdef{dshortest}, we can compute the decreasing rank distance between $u$ and $w$ via $v$ (line 4-5). Then we continue to explore next vertex $v$ (line 6) and add the new one into $V(\sdgu(u))$ (line 7).
 

\begin{algorithm}[htb]
        \caption{$\kw{KNN}\textrm{-}\kw{Index}\textrm{-}\kw{Ins}(G', u)$}
        \small
        \label{alg:insert}
        \DontPrintSemicolon            
            %\KwInput{\knnindex and a inserted vertex $u$}
            %\KwOutput{The updated \knnindex}
            	%construct $\sdgu(u)$ by conducting BFS search from $u$ on $G'$;\;
            	$v \gets u$; $V(\sdgu(u)) \gets \{v\}$; \;
            	$\psd[u,\cdot] \gets +\infty$; $\psd[u,u] \gets 0$;\;
            	\While{$|\keyU(v)| \neq 0$}{
            		%\For{$w \in \keyU(v)$}{
            			%$\psd[u,w] \gets \min\{ \phi((w,v),G') + \psd[u,v], \psd[u,w] \}$;
            		$d \gets \min_{w \in \keyU(v)}\{\phi((w,v),G') + \psd[u,v] \}$; \;
            		$\psd[u,w] \gets \min\{ \psd[u,w], d \}$; \;
            		%}
            		$v \gets argmin_{w \in \keyU(v)} \pi(w)$; \;
            		$V(\sdgu(u)) \gets V(\sdgu(u)) \cup \{v\}$; \;
            	}
            	%\For{\textbf{each} $v \in V(\sdgu(u))$ in increasing order of $\pi(v)$}{
            %    $v_k \gets$ the last vertex in $\pknnalg(v)$;\;
            %    \If{$\psd(v,v_k) > \psd[v]$}{
            %			remove $v_k$ from $\pknnalg(v)$; \;
            	%		insert $u$ into $\pknnalg(v)$; \;
            %   }
            	%}
\end{algorithm} 

\begin{theorem}
	Given the \sdg $G'$ of a road network $G$ and an inserted candidate object $u$, the time complexity of \refalg{insert} is $O(\eta \cdot \tau)$, where $\eta = \kw{max}_{v \in V(G)}|\sdgu(v)|$ and $\tau = \kw{max}_{v \in V(G)}|\keyU(v)|$.
\end{theorem}

\proofsketch
	The $\psd[u,\cdot]$ computation costs $O(\tau)$ time (line 4-5). Therefore, the total time complexity of \refalg{insert} is $O(\eta \cdot \tau)$.
\eop 

\stitle{Query after inserting objects} The algorithm for $q$'s $k$NN query after inserting an object $u$ is shown in \refalg{insert_tar}.
We first obtain the decreasing rank distance array, i.e, $\psd[u,\cdot]$, and $V(\sdgu(u))$ from \refalg{insert} (line 1). Then we initialize $v, V(\sdgu(q))$ and $\psd[q,\cdot]$ (line 2-3). Similarly, $\psd[q,\cdot]$ is an array to store the decreasing rank distance between $q$ and each vertex $v$ in $V(\sdgu(q)$, i.e, $\psd(u,v), v \in V(\sdgu(q)$. We calculate the decreasing rank distance (line 4-8). We calculate $\sd(q,u)$ (line 9-10). We use $q_k$ to denote the last vertex in $\knnalg(q)$ (line 11). We check whether the distance between $u$ and $q$ is shorter than the distance between $q_k$ and $q$ and then decide whether it needs to update $\knnalg(q)$ (line 12-14).

\begin{algorithm}[htb]
        %\caption{Query after Inserting Objects}
        \caption{$\kw{KNN}\textrm{-}\kw{Index}\textrm{-}\kw{Ins}(G, G', \knnalg(q), u, q)$}
        \label{alg:insert_tar}
        \small
        \DontPrintSemicolon            
            %\KwInput{\knn after inserting $u$ and a query vertex $v$}
            %\KwOutput{$\knnalg(v)$}
            	%Updated \knnindex and $UG(u)$ $\gets \refalg{insert}$; \;
            	%\If{$v \in V(UG(u))$}{
            	%	return $\knnalg(v)$; \;
            	%}            	
            %$UG(v) \gets$ the upper graph of $v$; $\sd(\cdot) \gets +\infty$; \;
            	%\If{$u \in V(UG(v))$}{
            	%	$v_k \gets$ the last vertex in $\knnalg(v)$;\;
            	%	\If{$dist(v,v_k) > dist(v,u)$}{
            	%		replace $v_k$ with $u$ in $\knnalg(v)$; \;
            	%	}
            %		return $\knnalg(v)$; \;            		
            	%}
            	%$\Omega \gets V(UG(u)) \cap V(UG(v))$; \;
            %$\sd(u,v) \gets \min_{w \in \Omega}\{\sd(u,w) + \sd(w,v)\}$; \;
            	%	$v_k \gets$ the last vertex in $\knnalg(u)$;\;
            	%	\If{$dist(v,v_k) > dist(v,u)$}{
            	%		replace $v_k$ with $u$ in $\knnalg(v)$; \;
            %		}
           %construct $\sdgu(q)$ by conducting BFS search from $q$ on $G'$;\;
           $\psd[u,\cdot]$ and $V(\sdgu(u)) \gets \kw{KNN}\textrm{-}\kw{Index}\textrm{-}\kw{Insert^*}(G', u)$; \; 
           $v \gets q$; $V(\sdgu(q)) \gets \{v\}$; \; 
           $\psd[q, \cdot] \gets +\infty$; $\psd[q, q] \gets 0$;\;
            	\While{$|\keyU(v)| \neq 0$}{
            		%\For{$w \in \keyU(v)$}{
            			%$d \gets \phi((w,v),G') + \psd[q,v] \}$; \;
            			%$\psd[q,w] \gets \min\{ \psd[q,w], d \}$; \;
            			%$\psd[w] \gets \min \{d, \psd[w] \}$; \;
            		%}
            		$d \gets \min_{w \in \keyU(v)}\{\phi((w,v),G') + \psd[u,v] \}$; \;
            		$\psd[u,w] \gets \min\{ \psd[u,w], d \}$; \;
            		$v \gets argmin_{w \in \keyU(v)} \pi(w)$; \;
            		$V(\sdgu(q)) \gets V(\sdgu(q)) \cup \{v\}$; \;
            	}
            %	$\sd(\cdot) \gets +\infty$; $\sd[q] \gets 0$;\;
            	%\For{\textbf{each} $v \in V(\sdgu(q))$ in decreasing order of $\pi(v)$}{
            		%$d \gets \min_{w \in \keyU(v)}\{ \phi((v,w),G')+ \sd[w] \}$; \;
            		%$\sd[v] \gets \min\{ d,\psd[v]\}$; \;
            		
            		%$v_k \gets$ the last vertex in $\knnalg(v)$; \;
            		%\If{$\sd(v,v_k) > \sd[v]$}{
            		%	remove $v_k$ from $\knnalg(v)$; \;
            		%	insert $u$ into $\knnalg(v)$; \;
            		%}
           %}
           $\mathcal{C} \gets V(\sdgu(u)) \cap V(\sdgu(q))$;\;
           $\sd(u,q) \gets \min_{w \in \mathcal{C}} \psd[u,w] + \psd[q,w]$; \;
           $q_k \gets$ the last vertex in $\knnalg(q)$; \;
           \If{$\sd(q,q_k) > \sd(u,q)$}{
            		remove $q_k$ from $\knnalg(q)$; \;
            		insert $u$ into $\knnalg(q)$; \;
            	}
            return $\knnalg(q)$;\;
\end{algorithm} 

\begin{theorem}
	Given the \sdg $G'$ and $\knnalg(\cdot)$ of a road network $G$, an inserted candidate object $u$ and a query vertex $q$, the time complexity of \refalg{insert_tar} is $O(\eta \cdot \tau)$, where $\eta = \kw{max}_{v \in V(G)}|\sdgu(v)|$ and $\tau = \kw{max}_{v \in V(G)}|\keyU(v)|$.
\end{theorem}

\proofsketch
	\refalg{insert} needs $O(\eta \cdot \tau)$ time (line 1). $\psd[q,\cdot]$ computation costs $O(\eta \cdot \tau)$ time (line 4-8). The intersection $V(\sdgu(u)) \cap V(\sdgu(q))$ is bounded by $\eta$, so the distance computation costs $\eta$ (line 9-10). Since $\knnalg(q)$ is stored in a bidirectional linked list, we can obtain the last vertex in $\knnalg(q)$ in  $O(1)$ time (line 11). Therefore, the total time complexity of \refalg{insert} is $O(\eta \cdot \tau)$.
\eop


%When answering a query after inserting an object into the candidate set $\mathcal{M}$, it is unnecessary to update \knn for vertices with higher rank than $v_q$, since many them are not queried. In \refsec{exp}, we will show the frequency that vertices can reuse updated \knn, which is very low. So we can skip the step of updating \knn for vertices with higher ranks than $v_q$, which means we only update $\knnalg(v_q)$. To update exact and accurate \knn, we need to calculate the global shortest distance between $v_q$ and $v_{in}$ and then to compare $dist(v_q,v_{in})$ with $dist(v_q,v_k)$ from original $\knnalg(v_q)$. $v_k$ represents $k$th vertex in $\knnalg(v_q)$. Only when $dist(v_q,v_{in}) < dist(v_q,v_k)$, we need to insert $v_{in}$ to an accurate position of $\knnalg(v_q)$ and then delete the final one vertex. Otherwise, $\knnalg(v_q)$ is the direct answer.
